ISO-SWS calibration and the accurate modelling of cool-star atmospheres - III. A0 to G2 stars

Vega, Sirius, Beta Leo, Alpha Car and Alpha Cen A belong to a sample of twenty stellar sources used for the calibration of the detectors of the Short-Wavelength Spectrometer on board the Infrared Space Observatory (ISO-SWS). While general problems with the calibration and with the theoretical modelling of these stars are reported in Decin et al. (2002), each of these stars is discussed individually in this paper. As demonstrated in Decin et al. (2002), it is not possible to deduce the effective temperature, the gravity and the chemical composition from the ISO-SWS spectra of these stars. But since ISO-SWS is absolutely calibrated, the angular diameter of these stellar sources can be deduced from their ISO-SWS spectra, which consequently yields the stellar radius (R), the gravity-inferred mass (M) and the luminosity (L) for these stars. These deduced parameters are confronted with other published values and the goodness-of-fit between observed ISO-SWS data and the corresponding synthetic spectrum is discussed.

==> h3318_mac.tex <==
%% file: rrmacros2e.tex = Rob Rutten's standard LaTeX macros
%% last: Apr 20 2000
%% site: ~/rr/dip/texdip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BIBTEX EXPLANATION
%% Use BibTeX with the proper JOURNAL.STY, BIB.STY and BIB.BST style files.
%% The required statement combinations sit in template files:
%%    RRPAPER.TPL, AAPAPER.TPL, APJPAPER.TPL, ESAPROC.TPL, KLUWER.TPL,
%%    SWANSONG.TPL, PASP.TPL etc.,  
%% linked to directory /rrtex/templates
%% My RJR-typed -.BIB files are linked to /rrtex/bibfiles/rjr/bib.
%% My ADS-copied -.BIB files are linked to /rrtex/bibfiles/ads/bib.
%% Journal abbreviations are specified in AAJOUR.BIB (A&A, APJ format) and
%%   in JOURNALS.BIB (classical longer format), both in /rrtex/styles.
%%   The ADS abbreviations are redefined below (also two formats).
%% To use bibtex use script rrbibtex (in ~rutten/bin).
%%
%% Cites:   \cite*{Rutten1990a}                        }      
%%               ==>  Rutten (1990)                    } for in-text
%%          \cite*{Gurtovenko+Kostik+Rutten1990b}      } references
%%               ==>  Gurtovenko et al. (1990)        }
%%          \cite{Rutten1990a}                       }
%%               ==>  Rutten 1990                    } for between (...)
%%          \cite{Gurtovenko+Kostik+Rutten1990b}     } references
%%               ==>  Gurtovenko et al. 1990          }
%%          (Rutten 1990a, 1990b)
%%                    \nocite{Rutten1990c}  
%%                    \nocite{Rutten1990f}
%%          NB: \nocite*{..} makes Bibtex produce ALL bibliography entries
%%          NB: Bibtex may mix up the order, putting a later paper
%%              before an earlier one even in the same journal, becauses it
%%              alphabetizes on title after authors.  If it bothers you
%%              then correct the final -.BBL file, or fix the problem
%%              by adding fake digits to TITLE fields in .BIB files 
%%              (see Jo Bruls' README_order with my -.BIB files).
%%
%% Full citations for publication lists and PRINTBIB:
%%              \fullreferences (adds full titles and end pages)
%% 
%% References:
%%          - RRBIB: \section*{References} \references 
%%          - FULLBIB: \section*{References} \fullreferences
%%          - AABIB: no section header, \aareferences
%%          - APJBIB: no section header, \apjreferences
%%          - KLUWBIB: no section header, \references
%%          - ESA: no BIB.STY, section header ESAPROC.TPL, \esareferences
%%          - set \parsep=0ex to delete blank lines between references
%%          - execute latex, rrbibtex, latex twice
%%          - for email/ftp transfer: comment \references statement out and
%%            merge the -.BBL file there instead, or ftp that as well.
%%            Also ftp or insert this macro file, and email/ftp xxxBIB.STY.
%%
%% Database printout: ps files under /rrtex/bibfiles
%%
%% ADS: As of July 1996 I use ADS entries.  I  pull XXX.BIB files over
%%      from ADS and also XXX.ABS files with the corresponding abstracts.  
%%      They sit in /rrtex/bibfiles/ads/bib and /rrtex/bibfiles/ads/abs.
%%      Script RRBIBTEX copies all the XXX.BIB files to a short-lived
%%      file /scratch/strknd/rutten/adsfiles.bib that is searched by BibTeX 
%%      (appropriate BibTeX path in my .login) from script RRBIBTEX.
%%      BibTeX may complain about repeated ADS entries; don't bother.
%% NB: don't refer to the same paper with both its ADS XXX.BIB label 
%%     and its old bibfile label - or you get that reference twice.
%%     Check the resulting reference list for such duplicates.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ADS journal abbreviations: long and short versions, also in RJR.BIB
\newcount\longrefs
\def\aap{\ifnum\longrefs=1 {Astron.\ Astrophys.}\else 
                           {A\hbox{\rm \&}A}\fi}
\def\aapr{\ifnum\longrefs=1 {Astron.\ Astrophys.\ Rev.}\else 
                            {A\hbox{\rm \&}AR}\fi}
\def\aaps{\ifnum\longrefs=1 {Astron.\ Astrophys.\ Suppl.}\else 
                            {A\hbox{\rm \&}AS}\fi}
\def\aj{\ifnum\longrefs=1 {Astron.\ J.}\else 
                          {AJ}\fi} 
\def\ao{\ifnum\longrefs=1 {Applied Optics}\else 
                           {Appl.\ Opt.}\fi} 
\def\aspcs{\ifnum\longrefs=1 {Astron.\ Soc.\ Pacific Conf. Series}\else 
                           {ASP Conf.\ Ser.}\fi} 
\def\apj{\ifnum\longrefs=1 {Astrophys.\ J.}\else 
                           {ApJ}\fi} 
\def\apjl{\ifnum\longrefs=1 {Astrophys.\ J. Lett.}\else 
                            {ApJ}\fi} 
\def\aplett{\ifnum\longrefs=1 {Astrophys.\ J. Lett.}\else 
                            {ApJ}\fi} 
\def\apjs{\ifnum\longrefs=1 {Astrophys.\ J. Suppl.}\else 
                            {ApJS}\fi}
\def\apss{\ifnum\longrefs=1 {Astrophys.\ and Space Science}\else 
                            {Ap\hbox{\rm \&}SS}\fi}
\def\araa{\ifnum\longrefs=1 {Ann.\ Rev.\ Astron.\ Astrophys.}\else 
                            {ARA\hbox{\rm \&}A}\fi}
\def\azh{\ifnum\longrefs=1 {Astronomicheskii Zhurnal}\else 
                            {Astron.\ Zhur.}\fi}
\def\baas{\ifnum\longrefs=1 {Bull.\ Am.\ Astron.\ Soc.}\else 
                            {BAAS}\fi}
\def\bain{\ifnum\longrefs=1 {Bull.\ Astronom.\ Institutes Netherlands}\else
                            {Bull.\ Astr.\ Inst.\ Neth.}\fi}
\def\gca{\ifnum\longrefs=1 {Geochim.\ Cosmochim.\ Acta}\else 
                           {Geochim.\ Cosmochim.\ Acta}\fi}
\def\grl{\ifnum\longrefs=1 {Geophys.\ Res.\ Lett.}\else 
                           {Geoph.\ Res.\ Lett.}\fi}
\def\iaucirc{\ifnum\longrefs=1 {IAU Circulars}\else 
                          {IAU Circ.}\fi}
\def\ip{\ifnum\longrefs=1 {in press}\else 
                          {in press}\fi}
\def\jgr{\ifnum\longrefs=1 {J.\ Geophys.\ Res.}\else 
                           {J.\ Geophys.\ Res.}\fi}  
\def\jrasc{\ifnum\longrefs=1 {J.\ Royal Astron.\ Soc.\ Canada}\else 
                           {JRAS Can.}\fi}  
\def\mnras{\ifnum\longrefs=1 {Mon.\ Not.\ Roy.\ Astron.\ Soc.}\else 
                             {MNRAS}\fi} 
\def\nat{\ifnum\longrefs=1 {Nature}\else 
                           {Nat}\fi}
\def\pasj{\ifnum\longrefs=1 {Pub.\ Astron.\ Soc.\ Japan}\else 
                            {PASJ}\fi} 
\def\pasp{\ifnum\longrefs=1 {Pub.\ Astron.\ Soc.\ Pacific}\else 
                            {PASP}\fi} 
\def\physscr{\ifnum\longrefs=1 {Physica Scripta}\else 
                            {Phys.\ Scrip.}\fi} 
\def\planss{\ifnum\longrefs=1 {Planetary \& Space Science}\else 
                            {Plan. \& Space Sci.}\fi} 
\def\procspie{\ifnum\longrefs=1 {Proc.\ SPIE}\else 
                            {Proc.\ SPIE}\fi} 
\def\qjras{\ifnum\longrefs=1 {Quarterly J.\ Royal Astron.\ Soc.}\else 
                            {QJRAS}\fi} 
\def\sa{\ifnum\longrefs=1 {Soviet Astron..}\else 
                               {Sov.\ Astron.}\fi}
\def\skytel{\ifnum\longrefs=1 {Sky \& Telescope}\else 
                            {Sky \& Tel.}\fi} 
\def\solphys{\ifnum\longrefs=1 {Solar Phys.}\else 
                               {Solar Phys.}\fi}
\def\ssr{\ifnum\longrefs=1 {Space Science Rev.}\else 
                               {Space\ Sci.\ Rev.}\fi}

%% bibfile specification
%\def\bibfiles{/home/leen/latex/bibtex/bibliofile}   %% bibfiles

%% \references (JOURNALS.BIB and AAJOUR.BIB sit in /rrtex/styles)
%\def\references{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/rrbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\aareferences{\longrefs=0  \bibliographystyle{/home/leen/latex/bibtex/aa}
%            \bibliography{/home/leen/latex/bibtex/aajour,\bibfiles}}
%\def\apjreferences{\longrefs=0  \bibliographystyle{/home/leen/latex/bibtex/apjbib}
%             \bibliography{/home/leen/latex/bibtex/ajour,\bibfiles}}
%\def\fullreferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/namebib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\nlreferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/nlbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\titlereferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/titlebib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\esareferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/esabib} 
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\kluwreferences{\longrefs=1 \bibliographystyle{/home/leen/latex/bibtex/kluwbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\kluwtitlereferences{\longrefs=1 \bibliographystyle{/home/leen/latex/bibtex/kluwtbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\natbibreferences{\longrefs=1 \bibliographystyle{/home/leen/latex/bibtex/natbib/plainnat}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INSTITUTE ADDRESS ABBREVIATIONS
\def\nl{,\ } %%\def\nl{\newline}  %% redefine as \newline for mail addresses
\def\AFGL{Air Force Geophysics Lab.\nl Sunspot NM~88349\nl USA}
\def\Arcetri{Osservatorio Astrofisico di Arcetri\nl Largo E. Fermi 5\nl
         I--50125 Firenze\nl Italy}
\def\Armagh{Armagh Observatory\nl College Hill\nl Armagh, BT61~9DG\nl
         Northern Ireland}
\def\ASTRON{Stichting ASTRON\nl Postbus 2\nl NL--7990~AA Dwingeloo\nl
         The Netherlands}
\def\Caltech{Solar Astronomy\nl 105--24 Caltech\nl 
         Pasadena, CA~91125\nl USA}
\def\Catania{Osservatorio Astrofisico di Catania\nl Viale A. Doria 6\nl 
         Citta Universitaria\nl I--95125 Catania\nl Italy}
\def\CfA{Center for Astrophysics\nl 60 Garden Street\nl 
         Cambridge, MA~02138\nl USA}
\def\CHEAF{CHEAF\nl Kruislaan 403\nl NL--1098~SJ Amsterdam}
\def\DAMTP{Dept.\ Applied Math.\ and Theor.\ Phys.\nl Silver Street\nl 
         Cambridge CB3~9EW\nl United Kingdom}
\def\Dwingeloo{Radio Sterrewacht Dwingeloo\nl Postbus 2\nl
      NL--7990 AA Dwingeloo\nl The Netherlands}
\def\ESA{European Space Agency\nl 8--10 Rue Mario Nikis\nl
         F--75738 Paris Cedex 15\nl France} 
\def\ESO{European Southern Observatory\nl Karl--Schwarzschild-Str. 2\nl 
         D--85748 Garching bei M\"unchen\nl Germany}
\def\ESTEC{ESA Space Science Department\nl ESTEC\nl 
         Postbus 299\nl NL--2200~AG Noordwijk\nl The Netherlands}
\def\ETH{Institute of Astronomy\nl ETH--Zentrum\nl 
         CH--8092 Z\"urich\nl Switzerland}
\def\Goddard{NASA Goddard Space Flight Center \nl Greenbelt, MD~20771\nl USA}
\def\Goettingen{Universit\"{a}ts Sternwarte\nl Geismarlandstrasse 11\nl
         D--37083 G\"{o}ttingen\nl Germany}
\def\HAO{High Altitude Observatory\nl NCAR\nl PO Box 3000\nl 
         Boulder, CO 80307--3000\nl USA}
\def\Hawaii{Institute for Astronomy\nl 2680 Woodlawn Drive\nl 
         Honolulu, HAWAII 96822\nl USA}
\def\IAC{Instituto de Astrof{\'{\i}}sica de Canarias\nl C/ Via Lactea S/N\nl
         E--38200 La Laguna, Tenerife\nl Spain}
\def\IAP{Institut d'Astrophysique de Paris\nl 98-bis Boulevard Arago\nl
         F--75014 Paris\nl France}
\def\JILA{Joint Inst.\ Lab.\ Astrophysics\nl Campus Box 440\nl 
         Univ.\ Colorado\nl Boulder CO 80309--0440\nl USA}
\def\JPL{Jet Propulsion Laboratory\nl 4800 Oak Grove Drive\nl
         Pasadena CA~91109\nl USA}
\def\Kiel{Institut f\"ur Theor.\ Physik und Sternwarte\nl 
         Olshausenstrasse 40\nl D--2300 Kiel 1\nl Germany}  %% postcode?
\def\Kiev{Main Astronomical Observatory\nl Academy of Sciences Ukraine\nl 
         Golosiiv\nl  Kyiv 22\nl  252650 Ukraine}
\def\KIS{Kiepenheuer Institut f\"ur Sonnenphysik\nl Sch\"oneckstrasse 6\nl
         D--79104 Freiburg\nl Germany} 
\def\KSW{Kapteyn Sterrewacht\nl Mensingheweg 20\nl NL--9301 KA Roden\nl
         The Netherlands} 
\def\LKBF{Secretaris/Pennningmeester LKBF\nl \RUL}
\def\LPARL{Lockheed Martin ATC\nl Solar \& Astrophysics Lab\nl 
         Org.\ H1--12, Bldg.\ 252\nl 3251 Hanover Street\nl 
         Palo Alto, CA~94304--1187\nl USA}
\def\Meudon{Observatoire de Paris\nl F--92195 Meudon Principal Cedex\nl 
         France}
\def\NJIT{Department of Physics and Mathematics\nl
          New Jersey Institute of Technology\nl University Heights\nl
          Newark NJ 07102\nl USA}
\def\NOAO{National Opt.\ Astron.\ Obs.\nl P.O. Box 26732\nl 
         Tucson AZ 85726--26732\nl USA}
\def\NRL{Naval Research Laboratory\nl 
         Washington DC 20376--5000\nl USA}   %?? code
\def\NSO{National Solar Observatory\nl PO Box 26732\nl 
         Tucson AZ 85726--6732\nl USA}       
\def\Orsay{Institute d'Astrophysique Spatiale\nl 
         Universit\'e Paris XI--CNRS\nl B\^atiment 121\nl 
         F--91405 Orsay\nl France}
\def\Oslo{Institute of Theoretical Astrophysics\nl 
         P.O. Box 1029, Blindern\nl N--0315 Oslo\nl Norway}  
\def\OAC{Osservatorio di Capodimonte\nl Via Moiariello 16\nl 
         I--80131 Napoli\nl Italy}
\def\Ondrejov{Astronomical Institute\nl CS--25165 Ondrejov\nl Czech Republic}
\def\Potsdam{Astrophysikalisches Institut\nl Sonnenobservatorium 
         Einsteinturm\nl Telegrafenberg\nl D--14473 Potsdam\nl Germany}
\def\Pulkovo{Pulkovo Observatory\nl Pulskoske Shsee 65--1\nl
         196140 St.\ Petersburg\nl Russia}
\def\RUG{Kapteijn Laboratorium\nl Postbus 800\nl NL--9700~AV Groningen\nl
         The Netherlands}
\def\RUL{Sterrewacht\nl Postbus 9513\nl NL--2300~RA Leiden\nl 
         The Netherlands}
\def\SIU{Sterrekundig Instituut\nl Postbus 80\,000\nl
         NL--3508 TA Utrecht\nl The Netherlands}
\def\SPO{NSO/Sacramento Peak\nl P.O. Box 62\nl 
         Sunspot, NM 88349--0062\nl USA}
\def\Stanford{Center for Space Science and Astrophysics\nl  ERL 328\nl 
         Stanford University\nl Stanford CA 94305--4055\nl  USA}
\def\SRON{SRON\nl Sorbonnelaan 2\nl NL--3584 CA Utrecht\nl The Netherlands}
\def\SRONRUG{SRON\nl Postbus 800\nl NL--9700~AV Groningen\nl 
         The Netherlands}
\def\Uppsala{Astronomiska Observatoriet\nl Box 515\nl S--75120 Uppsala\nl
         Sweden}
\def\UvA{Sterrekundig Instituut ``Anton Pannekoek''\nl Kruislaan 403\nl
         NL--1098~SJ Amsterdam\nl The Netherlands}
\def\VU{Afdeling Sterrekunde\nl Vrije Universiteit\nl De Boelelaan 1081\nl
         NL--1081 HV Amsterdam\nl The Netherlands}
\def\Wuerzburg{Institut f\"ur Astronomie und Astrophysik\nl  Am Hubland\nl
      D--97074 W\"{u}rzburg\nl Germany}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% from DUTCH.STY
\def\dutch{\def\refname{Referenties}\def\abstractname{Samenvatting}%
  \def\bibname{Bibliografie}\def\chaptername{Hoofdstuk}%
  \def\appendixname{Bijlage}\def\contentsname{Inhoudsopgave}%
  \def\listfigurename{Lijst van figuren}\def\listtablename{Lijst van tabellen}%
  \def\indexname{Index}\def\figurename{Figuur}\def\tablename{Tabel}%
  \def\partname{Deel}\def\enclname{Bijlage(n)}\def\ccname{Ter attentie van}%
  \def\headtoname{Aan}\def\headpagename{Pagina}%
  \def\today{\number\day\space\ifcase\month\or januari\or februari\or maart\or%
     april\or mei\or juni\or juli\or augustus\or september\or oktober\or%
     november\or december\fi \space\number\year}%
  \typeout{
              >>>>> use hlatex209 for Dutch hyphenation <<<<< 
         }}
\hyphenation{Schrij-ver Krij-ger Kuij-pers Bal-le-gooij-en}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% warningoverprint
%% eg: \warningoverprint{DRAFT}, or SUBMITTED, CONFIDENTIAL from Eric Bakker
\def\warningoverprint #1{\special{!userdict begin 
  /bop-hook{gsave 100 600 translate -45 rotate /Times-Roman findfont 
  100 scalefont setfont 0 0 moveto 0.9 setgray (#1) show grestore}def end}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% figures
%% journal figures, use templettes in AAFIGS.TPL, APJFIGS.TPL, MULTIFIG.TPL
\newcounter{onefig} \newcounter{fignumber}
\newcount\nocaptions \newcount\nofigures \newcount\figwidth
\newcount\viewgraphs
\def\figsfile{} \def\figspath{} \def\paper{} \def\format{} \def\figlabel{} 
\long\def\nextfig#1{\setcounter{figure}{\value{fignumber}}
  \addtocounter{fignumber}{1}
  \ifnum \viewgraphs=1 \newpage \pagestyle{empty} \fi 
  \ifnum\value{onefig}=0 #1 \fi                 
  \ifnum\value{onefig}=\value{fignumber} #1 \fi}
\def\figwidths#1#2{\ifnum \nocaptions=1 #2mm \else #1mm \fi}  
%%\def\capspace#1{\vspace{#1}}     %% A&A: redefine \capspace = \picplace{#1}
\def\paper#1{}  %% redefine for separate-figure identification line
\long\def\plotfig#1#2{\ifnum \nofigures=1 \else #2 \fi}
\long\def\captiontext#1{\ifnum \nofigures=1 \raggedright \fi 
   \ifnum \nocaptions=1 \paper
     \ifnum \viewgraphs=0 
       \newline  \mbox{}\hrulefill\mbox{} \newline 
       \newline label:~\{\figlabel\} 
     \fi 
%%   \else \ifnum \nofigures=0 \{\figlabel\}~~ \fi   %% adds label
     \else \ifnum \nofigures=0 \fi 
   #1 \fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MULTI-FILE FIGURE
%% macros to combine separate postscript files into one multi-panel figure;
%% templettes in template files AAFIGS.TPL, APJFIGS.TPL, MULTIFIG.TPL.
%% - measure panel bounding boxes with GHOSTVIEW
%%   - large lower-left (outside axis labels)
%%   - small lower-left (between labels and numbers or just outside frame)
%%   - upper-left
%% - use \barepanel, \labelxpanel, \labelypanel, \labelxypanel 
%%   to control layout, for example to cut all x labels off and replace
%%   by single full-width LaTeX x label.  See templettes or test files.
%%   First specify \panelsize; \panelheight=0 maintains frame aspect ratio.
\newcount\panelwidth \newcount\panelheight 
\newcount\bxmin \newcount\bymin \newcount\bxmax \newcount\bymax
\newcount\tbxmin \newcount\tbymin
\newcount\tpanelwidth \newcount\tpanelheight \newcount\tpdif
\panelwidth=70 \panelheight=70  %% defaults (mm)
\def\panelsize #1,#2;{\panelwidth=#1 \panelheight=#2}  
     %% units MUST be mm; \panelheight=0 maintains frame aspect ratio
\def\setbb #1,#2;#3,#4;#5,#6;{% UNITS: bp (from ghostview)
  \tbxmin=#1 \tbymin=#2    %% full box (axis titles) lower left corner
  \bxmin=#3 \bymin=#4      %% bare box (ticks only) lower left corner
  \bxmax=#5 \bymax=#6}     %% upper right corner
\def\barepanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \epsfig{file=#1,%
     bbllx=\bxmin bp,bblly=\bymin bp,bburx=\bxmax bp,bbury=\bymax bp,clip=,%
     width=\panelwidth mm,height=\tpanelheight mm}}
\def\labelypanel #1{% TeX permits only integer arithmetic, so bp and mm
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \tpdif=\bxmax \advance\tpdif by -\tbxmin
  \tpanelwidth=\panelwidth \multiply \tpanelwidth by \tpdif
  \tpdif=\bxmax \advance\tpdif by -\bxmin
  \divide \tpanelwidth by \tpdif
  \epsfig{file=#1,%
    bbllx=\tbxmin bp,bblly=\bymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=,width=\tpanelwidth mm,height=\tpanelheight mm}}
\def\labelxpanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \tpdif=\bymax \advance\tpdif by -\tbymin
  \multiply \tpanelheight by \tpdif
  \tpdif=\bymax \advance\tpdif by -\bymin
  \divide \tpanelheight by \tpdif
  \epsfig{file=#1,%
    bbllx=\bxmin bp,bblly=\tbymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=,width=\panelwidth mm,height=\tpanelheight mm}}
\def\labelxypanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \tpdif=\bxmax \advance\tpdif by -\tbxmin
  \tpanelwidth=\panelwidth \multiply \tpanelwidth by \tpdif
  \tpdif=\bxmax \advance\tpdif by -\bxmin
  \divide \tpanelwidth by \tpdif 
  \tpdif=\bymax \advance\tpdif by -\tbymin 
  \multiply \tpanelheight by \tpdif
  \tpdif=\bymax \advance\tpdif by -\bymin
  \divide \tpanelheight by \tpdif
  \epsfig{file=#1,%
    bbllx=\tbxmin bp,bblly=\tbymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=,width=\tpanelwidth mm,height=\tpanelheight mm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% panel label
%% adds labels to panels, from Louis Strous
%% eg \panellabel{1.5em}{0.5em}{(a)} = 1.5em from right, 0.5em from bottom
\newcommand{\panellabel}[3]{\makebox[0pt][r]{\raisebox{#2} #3 \hspace{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% float params
\def\topfraction{0.99}                      %% to permit many large figures
\def\dbltopfraction{0.99}
\def\textfraction{0.01} 
\def\floatpagefraction{0.99}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTS
%% Option for yes/no printing of internal comments within LaTeX output.
%% - Begin comment with new line with %CC 
%% - start each comment line with %, for example with %RR
%% - end comment with new line with %EE and blank line if paragraph end.
%% - example:
%%      %CC
%%      %RR This is a RR comment to his co-authors
%%      %EE
%%
%% For comment printing replace with editor everywhere (after the
%% \begin{document} command):
%%        %CC by \CC 
%%        %EE by \end{verbatim} \EE          
%% and change these back again for skipping comments in LaTeX printout.
%% The other text will be compressed when comments are printed.
%%
%% Skip comments permanently by taking out CC and EE lines. 
%% Don't delete comments if you wish to record evolutionary thinking.  
%%
\def\CC{\par \vspace*{-2ex} \footnotesize \baselineskip=8pt \begin{verbatim}}
\def\EE{\par \vspace*{-2ex} \normalsize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% IGNORE
\long\def\startignore #1\stopignore{}   %% use \startignore....\stopignore

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FULLFIGURE
%% for full-page figure with LaTeX caption use (Mats):
%%      \begin{figure}[p]
%%            \vbox to \textheight{\hbox{}\vfill
%%                  \caption[..]{\it............
%%                               \label{.....}}}
%%      \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TASK
\newenvironment{task}{%
  \begin{list}{$\bullet$}{\itemsep=1ex \parindent=3ex \parskip=1ex 
    \topsep=0ex}}
  {\end{list}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAMERA-READY ARTICLE HEADER
%% use for example: 
%%      \begin{koprr}
%%              {\large \bf  TITLE}\\[2ex]
%%              {\bf  AUTHORS}\\[2ex]
%%              {\sl  ADRRESS}\\[3cm]
%%      \end{koprr}
%%
\def\koprr{\list{}{      
  \itemindent=0pt \listparindent=0pt \itemsep=0pt
  \leftmargin=5ex}\item[]}                     %% 5ex = left margin
  \let\endkoprr=\endlist

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURETTE COLUMN
%% Blank column on the right for small figures.  Example: Seattle review
%% See also TeX parshape command and FLOATFIG style
%%
\def\kolom{\list{}{\rightmargin=5cm      %% 5cm = width column at right
  \topsep=0ex \itemsep=0cm \parsep=0ex \parskip=0ex \partopsep=0ex 
  \listparindent=3ex
  \itemindent=0pt \leftmargin=0pt} \item[] 
  \vspace*{-0ex}}                        %% this funny command kills gaps
  \let\endkolom=\endlist

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LIST PARAMETERS
\renewcommand{\labelitemi}{{\bf --}}                %% no bullets but dashes
\def\setlistparams{         
  \topsep=0.7ex                 %% ADAPT: parskip=0: 0.7;  parskip=1: -1.2ex
  \itemsep=0.7ex                %% space between items
  \leftmargini=3ex}             %% dashes at beginning of line 
\setlistparams                  %% recall after type changes 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALPHABETIC LIST
\newcounter{alistindex}  \newcounter{alistvalue}     %% problems: a)  b) etc
\newenvironment{alist}{%
   \begin{list}{\alph{alistindex})}{\usecounter{alistindex}}
   \itemsep=1.5ex \parskip=1ex}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LINE SPACING
\def\spacing #1{\small \renewcommand{\baselinestretch}{#1}
                \normalsize \setlistparams}             %% eg: \spacing{1.5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNINDENTED ITEMIZE
%% puts dashes fully left, no extra indent.  As ENUMERR below.
\newenvironment{itemrr}{\vspace*{-\parskip}
  \leftmargini=3ex \topsep=0.6ex       
  \begin{itemize}
     \itemsep=0.5ex \parindent=0ex \parsep=0ex}{
  \end{itemize} \vspace*{-\parskip}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONDENSED ITEMIZE
%% puts dashes fully left, no extra indent, small top and bottom spacing
%%                                   Example: Solar Physics Newsletter 3
\newenvironment{conditem}{               
  \leftmargini=6ex \topsep=0.2ex 
  \begin{itemize}
     \itemsep=0ex \parindent=3ex \parsep=0ex}{
  \end{itemize}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNINDENTED ENUMERATE
%% puts numbers fully left, no extra indent.  Example: Kiev IAU Summary
\newenvironment{enumerr}{               
  \leftmargini=3ex \topsep=1.5ex       
  \begin{enumerate}
     \itemsep=0.7ex \parindent=3ex \parsep=0ex}{
  \end{enumerate}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONDENSED ENUMERATE
%% puts numbers fully left, no extra indent, small top and bottom spacing.
%% Example: Solar Physics Newsletter 2 Huber item
\newenvironment{condenum}{               
  \leftmargini=3ex \topsep=0.5ex 
  \begin{enumerate}
     \itemsep=0ex \parindent=3ex \parsep=0ex}{
  \end{enumerate}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROMAN ENUMERATE
%% puts numbers fully left, uses (i), (ii), (iii) etc.                 
\newcounter{romenumnr}
\newenvironment{romanenum}{
  \leftmargini=5ex \topsep=1.5ex
  \begin{list}{(\roman{romenumnr}) --}{\usecounter{romenumnr}
      \itemsep=1ex \listparindent=3ex \parsep=0ex}}{
  \end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% POSTER PAGE
%% one page, shadowframe, large sansserif, for POSTER.TPL
%% usage: \posterpage{header}{text}  
%%        suppress header with {\mbox{}}
%%        text may contain titles, multiple paragraphs, item lists etc.
\newcommand{\posterpage}[2]{{\Large \sf \newpage
  \setlength{\minipagewidth}{\textwidth} \addtolength{\minipagewidth}{-2cm}
  \fboxrule=0.3ex \fboxsep=0ex
  \def\shadowparams{\topsep=-2.5ex \itemsep=-1.5ex \leftmargini=5ex}
  \renewcommand{\labelitemi}{$\bullet$}
  \parskip=3ex \shadowparams
  \savebox{\boxcontent}[\textwidth]{
    \begin{minipage}[t]{\minipagewidth}
        \parskip=3ex \vspace*{1ex}
        \begin{center} \LARGE \bf #1 \end{center} 
        \vspace{2ex} #2 \vspace*{3ex} \mbox{ }
    \end{minipage}}
  \hspace*{\textwidth} \hspace*{-0.8ex} \rule{2ex}{\dp\boxcontent}
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.2ex}
  \framebox[\textwidth]{\usebox{\boxcontent}}
  \par \vspace*{-3.0ex} \hspace*{1.7ex} \rule{\textwidth}{2ex}
  \setlistparams \renewcommand{\labelitemi}{{\bf --}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VWGRAPH
%% usage: \vwgraph{width}{header}{text}  
%%        suppress header with: \vwgraph{\mbox{}}{text} 
%%        specify fonts, eg: \vwgraph{\huge \bf ...}{\Large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\newcommand{\vwgraph}[3]{\newpage
    \begin{center}
     \shadowframe{#1}{
       \begin{center}
         \vspace*{2ex}
         {\Large \bf #2}\\[4ex]
       \end{center}
       {\Large \sf #3}}   %% ADAPT font
     \end{center}}
\newenvironment{itemvg}{
  \leftmargini=3ex \topsep=0.5ex
  \begin{itemize} \vspace{-1ex}
     \itemsep=0.5ex \parindent=3ex \parsep=0ex}{
  \end{itemize}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LECTVW
%% usage: \lectvw{header}{text}  = \vwgraph without shadow box
%%        suppress header with: \vwgraph{\mbox{}}{text} 
%%        specify fonts, eg: \vwgraph{\huge \bf ...}{\Large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\long\def\lectvw#1#2{\newpage \vspace*{-15mm}
    \begin{center}
       \begin{center}
         {\LARGE \sc \underline{#1}}\\[4ex]
       \end{center}
       {\Large \sf #2}   %% ADAPT font
     \end{center}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SHADOWFRAME
%% minipage in shadowframe, used in VWGRAPH.TPL 
%% usage: \shadowframe{width}{text}
%%        eg: \shadowframe{15cm}{\large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\newlength{\minipagewidth}
\newcommand{\shadowframe}[2]{
  \setlength{\minipagewidth}{#1} \addtolength{\minipagewidth}{-1cm}
  \fboxrule=0.5ex \fboxsep=0ex
  \def\shadowparams{\topsep=-2.5ex \itemsep=-1.5ex \leftmargini=5ex}
  \renewcommand{\labelitemi}{$\bullet$}
  \parskip=3ex \shadowparams 
  \savebox{\boxcontent}[#1]{         
    \begin{minipage}[t]{\minipagewidth}
      \vspace*{1.5ex} #2 \vspace*{0.5ex} \mbox{ } 
    \end{minipage}}
  \hspace*{#1} \hspace*{1.0ex} \rule{2ex}{\dp\boxcontent}  
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.9ex} 
  \framebox[#1]{\usebox{\boxcontent}}  
  \par \vspace*{-3.0ex} \hspace*{4.5ex} \rule{#1}{2ex}
  \setlistparams \renewcommand{\labelitemi}{{\bf --}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OVALHEAD
%% header in centered oval, 3 widths (8cm, 12cm, 16cm), for VWGRAPH.TPL
%% usage: \ovalhead{text}     eg: \ovalhead{\Large \bf Conclusions}
%%        \ovalhead{\mbox{}} suppresses oval
\newsavebox{\boxcontent}
\newcommand{\ovalhead}[1]{
  \unitlength=1cm
  \sbox{\boxcontent}{\mbox{~~{#1}~~}}
  \begin{center}
    \ifdim\wd\boxcontent>6ex 
    \ifdim\wd\boxcontent<8cm 
    \begin{picture}(8,3) \thicklines     
      \put(4.0,0.8){\oval(8,1.6)} 
      \put(0.0,0.7){\parbox{8cm}{
         \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \else \ifdim\wd\boxcontent<12cm 
    \begin{picture}(12,3) \thicklines     
        \put(6.0,0.8){\oval(12,1.6)} 
        \put(0.0,0.7){\parbox{12cm}{
           \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \else
    \begin{picture}(16,3) \thicklines     
        \put(8.0,0.8){\oval(16,1.6)} 
        \put(0.0,0.7){\parbox{16cm}{
           \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \fi \fi \fi
  \end{center}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COLLOQFRAME
%% shadowed frame, for colloquium and lunch talk announcements
%% use: \colloqframe{width}{text}
\newcommand{\colloqframe}[2]{
  \setlength{\minipagewidth}{#1} \addtolength{\minipagewidth}{-1cm}
  \fboxrule=0.5ex \fboxsep=0ex
  \parskip=3ex
  \savebox{\boxcontent}[#1]{
    \begin{minipage}[t]{\minipagewidth}
      \vspace*{1.5ex} #2 \vspace*{0.5ex} \mbox{ }
    \end{minipage}}
  \hspace*{#1} \hspace*{-0.8ex} \rule{2ex}{\dp\boxcontent}
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.9ex}
  \framebox[#1]{\usebox{\boxcontent}}
  \par \vspace*{-3.0ex} \hspace*{1.7ex} \rule{#1}{2ex}
  \renewcommand{\labelitemi}{{\bf --}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SOL OVAL
%% Old Utrecht sol symbol in label oval for SIU announcement labels 
%% Use: \soloval{text}
\newcommand{\soloval}[1]{\fboxrule=0.5mm \unitlength=1cm
\hspace*{5mm} \sol{20mm}\\[-20mm]
\begin{picture}(15,3) \thicklines
 \put(7.5,2){\oval(15.60,3.60)} \put(7.5,2){\oval(15.55,3.55)}
 \put(7.5,2){\oval(15.50,3.50)} \put(7.5,2){\oval(15.45,3.45)}
 \put(7.5,2){\oval(15.40,3.40)} \put(7.5,2){\oval(15.35,3.35)}
 \put(7.5,2){\oval(15.00,3.00)} \put(2.0,1.9){\parbox{13cm}{#1}}
\end{picture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION NUMBERING DEPTH
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTIONRR COMMANDS
                             %% use these for parskip>0 and/or to set labels
\def\chapterrr#1{\chapter{#1} \label{chap:#1} \vskip-\parskip}  
\def\sectionrr#1{\section{#1} \label{sec:#1} \vskip-\parskip}
\def\subsectionrr#1{\subsection{#1} \label{sec:#1} \vskip-\parskip}
\def\subsubsectionrr#1{\subsubsection{#1} \label{sec:#1}  \vskip-\parskip}
\def\paragraphrr#1{\paragraph{#1.} \label{sec:#1} \vskip-\parskip}
                                                     %% #1 without period

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SMALL SECTION HEAD 
\def\smallhead #1{\vspace{2ex} \noindent {\bf #1}~~~\noindent} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAMERA-READY SECTION HEADS
%% Alternative section heads for camera-ready output.
%% Use:    blank line + \head{SECTION HEADER} + blank line
%%         blank line + \subhead{Subsection Header} + blank line 
%%         blank line + \subsubhead{Subsubsection Header} + blank line
%% Note: often usage of e.g. \subsubsection*{3. Results} is better to
%%       obtain a smaller header since this won't occur at page bottom
\newcounter{headnr}            
\newcounter{subheadnr}[headnr]
\newcounter{subsubheadnr}[subheadnr]
\def\head #1\par{
  \stepcounter{headnr}                          %% sets subheadnr = 0 too 
  \vspace{2ex} \noindent                        %% 2ex = space above, no *
  {\bf \theheadnr~~~~#1}\\[1ex] \noindent}      %% 1ex = space below
\def\subhead #1\par{  
  \stepcounter{subheadnr}
  \vspace{1.3ex} \noindent
  {\bf \theheadnr.\arabic{subheadnr}~~~#1}\\[0.3ex] \noindent}
\def\subsubhead #1\par{
  \stepcounter{subsubheadnr}
  \vspace{1.0ex} \noindent
  {\bf \theheadnr.\arabic{subheadnr}.\arabic{subsubheadnr}~~~#1}\\ \noindent}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPS-EPS NEWSLETTER MACROS 
\def\epstitle #1{\parskip=0ex \vspace{-2ex}
          \subsubsection*{\center \framebox[8.5cm]{\large \bf #1}}
          \parindent=3ex \parskip=0ex}
\def\epsdoubletitle #1#2{\parskip=0ex \vspace{-2ex}
          \subsubsection*{\center {\large \sc #1}}
          \vspace{-0.3ex}
          {\center \framebox[8.5cm]{\large \bf #2}\\[1ex]}
          \parindent=3ex \parskip=0ex \noindent}
\def\epssmalltitle #1{\subsubsection*{
        \vspace{-5ex} \center {\normalsize \sl #1}} \vspace*{-1.0ex}}
\def\epsauthor #1{\par\vspace*{0.3ex} \hspace*{\fill}{\sl#1}\\}
\def\epsinst #1{\hspace*{\fill}{\small#1}\\}
\def\sigrjr{\hspace{1.5cm} \raisebox{-1.5cm}{%
  \epsfig{file=/f4-usr1/rutten/adm/letters/figs/rjr.ps,%
     bbllx=75bp,bblly=300bp,bburx=480bp,bbury=500bp,clip=,%
     angle=-5,width=4cm}} \vspace*{-1.2cm} \par}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DROPCAP
%%  big "miniature" from DROP.STY from Eric Bakker, use \dropcap{T}he
\font\dropfont= cmr12 scaled \magstep5
\def\dropcap#1#2{{\noindent
    \setbox0\hbox{\dropfont #1}\setbox1\hbox{#2}\setbox2\hbox{(}%
    \count0=\ht0\advance\count0 by\dp0\count1\baselineskip
    \advance\count0 by-\ht1\advance\count0by\ht2
    \dimen1=.5ex\advance\count0by\dimen1\divide\count0 by\count1
    \advance\count0 by1\dimen0\wd0
    \advance\dimen0 by.25em\dimen1=\ht0\advance\dimen1 by-\ht1
    \global\hangindent\dimen0\global\hangafter-\count0
    \hskip-\dimen0\setbox0\hbox to\dimen0{\raise-\dimen1\box0\hss}%
    \dp0=0in\ht0=0in\box0}#2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HANGLINE
%% next line indentation.  Usage: \hangline{2ex}.  End last with paragraph
\def\hangline #1{\parskip=0pt\par\noindent\hangafter=1\hangindent=#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LATIN ABBREVIATIONS
\def\rmit#1{{\it #1}}              %% italics (RR style, Kluwer)
                                   %% redefine for A&A and ApJ, no italics
\def\etal{\rmit{et al.}}           %% use \etal\ for space behind it        
\def\etc{\rmit{etc.}}           
\def\ie{\rmit{i.e.,}}              %% , required (Webster 1681)
\def\eg{\rmit{e.g.,}}              %% , required (Webster 1681)
\def\cf{cf.}                       %% no Latin, always Roman (Webster 1686)
\def\viz{\rmit{viz.}}
\def\vs{\rmit{vs.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPECTRA
\def\specchar#1{\uppercase{#1}}    %% to be redefined for A&A, small caps
\def\AlI{\mbox{Al\,\specchar{i}}}  %% \def, not \newcommand, for overwrites 
\def\BI{\mbox{B\,\specchar{i}}}    %% use \AlI\ for space behind it
\def\BII{\mbox{B\,\specchar{ii}}}  
\def\BaI{\mbox{Ba\,\specchar{i}}}  
\def\BaII{\mbox{Ba\,\specchar{ii}}} 
\def\CI{\mbox{C\,\specchar{i}}} 
\def\CII{\mbox{C\,\specchar{ii}}} 
\def\CIII{\mbox{C\,\specchar{iii}}} 
\def\CIV{\mbox{C\,\specchar{iv}}} 
\def\CaI{\mbox{Ca\,\specchar{i}}} 
\def\CaII{\mbox{Ca\,\specchar{ii}}} 
\def\CaIII{\mbox{Ca\,\specchar{iii}}} 
\def\CoI{\mbox{Co\,\specchar{i}}} 
\def\CrI{\mbox{Cr\,\specchar{i}}} 
\def\CrII{\mbox{Cr\,\specchar{ii}}} 
\def\CsI{\mbox{Cs\,\specchar{i}}} 
\def\CsII{\mbox{Cs\,\specchar{ii}}} 
\def\CuI{\mbox{Cu\,\specchar{i}}} 
\def\FeI{\mbox{Fe\,\specchar{i}}} 
\def\FeII{\mbox{Fe\,\specchar{ii}}} 
\def\FeXVI{\mbox{Fe\,\specchar{xvi}}}
\def\FrI{\mbox{Fr\,\specchar{i}}}
\def\HI{\mbox{H\,\specchar{i}}} 
\def\HII{\mbox{H\,\specchar{ii}}} 
\def\Hmin{\hbox{\rmH$^{^{_-}}\!$}}      %% H^min, very elegant
\def\Hemin{\hbox{{\rm He}$^{^{_-}}$}}    %% He^min, idem
\def\HeI{\mbox{He\,\specchar{i}}} 
\def\HeII{\mbox{He\,\specchar{ii}}} 
\def\HeIII{\mbox{He\,\specchar{iii}}} 
\def\KI{\mbox{K\,\specchar{i}}} 
\def\KII{\mbox{K\,\specchar{ii}}} 
\def\KIII{\mbox{K\,\specchar{iii}}} 
\def\LiI{\mbox{Li\,\specchar{i}}} 
\def\LiII{\mbox{Li\,\specchar{ii}}} 
\def\LiIII{\mbox{Li\,\specchar{iii}}} 
\def\MgI{\mbox{Mg\,\specchar{i}}} 
\def\MgII{\mbox{Mg\,\specchar{ii}}} 
\def\MgIII{\mbox{Mg\,\specchar{iii}}} 
\def\MnI{\mbox{Mn\,\specchar{i}}} 
\def\NI{\mbox{N\,\specchar{i}}}
\def\NaI{\mbox{Na\,\specchar{i}}}
\def\NaII{\mbox{Na\,\specchar{ii}}}
\def\NaIII{\mbox{Na\,\specchar{iii}}} 
\def\NiI{\mbox{Ni\,\specchar{i}}} 
\def\NiII{\mbox{Ni\,\specchar{ii}}}
\def\NiIII{\mbox{Ni\,\specchar{iii}}} 
\def\OI{\mbox{O\,\specchar{i}}} 
\def\OVI{\mbox{O\,\specchar{vi}}}
\def\RbI{\mbox{Rb\,\specchar{i}}} 
\def\RrI{\mbox{Rr\,\specchar{i}}}      %% Robruttenium I
\def\RrII{\mbox{Rr\,\specchar{ii}}}    %% Robruttenium II
\def\RrIII{\mbox{Rr\,\specchar{iii}}}  %% Robruttenium III
\def\SII{\mbox{S\,\specchar{ii}}} 
\def\SiI{\mbox{Si\,\specchar{i}}} 
\def\SiII{\mbox{Si\,\specchar{ii}}} 
\def\SrI{\mbox{Sr\,\specchar{i}}}
\def\SrII{\mbox{Sr\,\specchar{ii}}}
\def\TiI{\mbox{Ti\,\specchar{i}}} 
\def\TiII{\mbox{Ti\,\specchar{ii}}} 
\def\TiIII{\mbox{Ti\,\specchar{iii}}} 
\def\TiIV{\mbox{Ti\,\specchar{iv}}} 
\def\VI{\mbox{V\,\specchar{i}}} 
\def\HtwoO{\mbox{H$_2$O}}        %% H2O
\def\Otwo{\mbox{O$_2$}}          %% O2

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LINES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% hydrogen
\def\Halpha{\mbox{H$\alpha$}}           %% use \Halpha\ for space behind it
\def\Ha{\mbox{H$\alpha$}}
\def\Hbeta{\mbox{H$\beta$}}
\def\Hepsilon{\mbox{H$\epsilon$}}
\def\Bacont{\mbox{Ba\,{\small cont}}}
\def\Lyalpha{\mbox{Ly$\,\alpha$}}
\def\Lybeta{\mbox{Ly$\,\beta$}}
\def\Lycont{\mbox{Ly\,{\small cont}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Na D
\def\NaD{\mbox{Na\,\specchar{i}\,D}}    %% use \NaD\ for space behind it
\def\NaDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\NaID{\mbox{Na\,\specchar{i}\,\,D}}
\def\NaIDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaIDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\Done{\mbox{D$_1$}}
\def\Dtwo{\mbox{D$_2$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Mg b
\def\Mgbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\Mgbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\Mgbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}
\def\MgIb{\mbox{Mg\,\specchar{i}\,b}}
\def\MgIbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\MgIbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\MgIbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ca II H & K 
\def\CaIIK{\mbox{Ca\,\specchar{ii}\,\,K}}       %% use \CaIIK\ for space
\def\CaIIH{\mbox{Ca\,\specchar{ii}\,\,H}}
\def\CaIIHK{\mbox{Ca\,\specchar{ii}\,\,H\,\&\,K}}
\def\HK{\mbox{H\,\&\,K}}
\def\Kthree{\mbox{K$_3$}}      %% numbers not permitted, dammit
\def\Hthree{\mbox{H$_3$}}
\def\Ktwo{\mbox{K$_2$}}
\def\Htwo{\mbox{H$_2$}}
\def\Kone{\mbox{K$_1$}}     
\def\Hone{\mbox{H$_1$}}     
\def\KtwoV{\mbox{K$_{2V}$}}
\def\KtwoR{\mbox{K$_{2R}$}}
\def\KoneV{\mbox{K$_{1V}$}}
\def\KoneR{\mbox{K$_{1R}$}}
\def\HtwoV{\mbox{H$_{2V}$}}
\def\HtwoR{\mbox{H$_{2R}$}}
\def\HoneV{\mbox{H$_{1V}$}}
\def\HoneR{\mbox{H$_{1R}$}}
\def\Kg{{\KtwoV\ grain}}
\def\Kgs{{\KtwoV\ grains}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Mg II h & k 
\def\hk{\mbox{h\,\&\,k}}
\def\kthree{\mbox{k$_3$}}    
\def\hthree{\mbox{h$_3$}}
\def\ktwo{\mbox{k$_2$}}
\def\htwo{\mbox{h$_2$}}
\def\kone{\mbox{k$_1$}}     
\def\hone{\mbox{h$_1$}}     
\def\ktwoV{\mbox{k$_{2V}$}}
\def\ktwoR{\mbox{k$_{2R}$}}
\def\koneV{\mbox{k$_{1V}$}}
\def\koneR{\mbox{k$_{1R}$}}
\def\htwoV{\mbox{h$_{2V}$}}
\def\htwoR{\mbox{h$_{2R}$}}
\def\honeV{\mbox{h$_{1V}$}}
\def\honeR{\mbox{h$_{1R}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ATOMIC LEVEL
%% use:    \level 3s3p 3Pe
%%         \level 3s$^2$ {1,3}P{e,o}
%%         \level {} 3Ge
%%
\def\level #1 #2#3#4{$#1 \: ^{#2} \mbox{#3} ^{#4}$}   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STAR NAME
\newcommand{\starname}[2]{${#1}$\,{\rm {#2}}}  %% \starname{\alpha}{Cen~A} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROMAN CHARACTERS FOR MATH 
\def\rma{{\rm a}} \def\rmA{{\rm A}}             %% without space 
\def\rmb{{\rm b}} \def\rmB{{\rm B}}             %% use for indices etc. 
\def\rmc{{\rm c}} \def\rmC{{\rm C}} 
\def\rmd{{\rm d}} \def\rmD{{\rm D}} 
\def\rme{{\rm e}} \def\rmE{{\rm E}} 
\def\rmf{{\rm f}} \def\rmF{{\rm F}} 
\def\rmg{{\rm g}} \def\rmG{{\rm G}} 
\def\rmh{{\rm h}} \def\rmH{{\rm H}} 
\def\rmi{{\rm i}} \def\rmI{{\rm I}} 
\def\rmj{{\rm j}} \def\rmJ{{\rm J}} 
\def\rmk{{\rm k}} \def\rmK{{\rm K}} 
\def\rml{{\rm l}} \def\rmL{{\rm L}} 
\def\rmm{{\rm m}} \def\rmM{{\rm M}} 
\def\rmn{{\rm n}} \def\rmN{{\rm N}} 
\def\rmo{{\rm o}} \def\rmO{{\rm O}} 
\def\rmp{{\rm p}} \def\rmP{{\rm P}} 
\def\rmq{{\rm q}} \def\rmQ{{\rm Q}} 
\def\rmr{{\rm r}} \def\rmR{{\rm R}} 
\def\rms{{\rm s}} \def\rmS{{\rm S}} 
\def\rmt{{\rm t}} \def\rmT{{\rm T}} 
\def\rmu{{\rm u}} \def\rmU{{\rm U}} 
\def\rmv{{\rm v}} \def\rmV{{\rm V}} 
\def\rmw{{\rm w}} \def\rmW{{\rm W}} 
\def\rmx{{\rm x}} \def\rmX{{\rm X}} 
\def\rmy{{\rm y}} \def\rmY{{\rm Y}} 
\def\rmz{{\rm z}} \def\rmZ{{\rm Z}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNITS
\def\deg{\hbox{$^\circ$}}       %% \def for overwriting, \box for math
\def\degree{\hbox{$^\circ$}}
\def\degrees{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\bgmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\secarc{\hbox{$^{\prime\prime}$}}
\def\bgsec{\hbox{$^{\prime\prime}$}}
\def\kms{\hbox{km$\;$s$^{-1}$}}
\def\micron{\hbox{$\mu$m}}
\def\kayser{\hbox{$\rm cm^{-1}$}}
\def\Mxcm{\hbox{Mx\,cm$^{-2}$}}    %% no 2, damn tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VARIA
\def\dif{\: {\rm d}}                       %% differential d with space
\def\ep{\:{\rm e}^}                        %% e^ with space and roman e
\def\lambdop{\hbox{$\bf \Lambda$}}         %% plain Lambda operator

\def\gf{\mbox{$g \! f$}}                   %% \gf\ for space behind it

\def\ko{($k, \omega$)}                     %% k - omega 
\def\komega{($k, \omega$)}                 %% k - omega 
\def\VminI{\hbox{$V\!\!-\!\!I$}}           %% V-I
\def\IminI{\hbox{$I\!\!-\!\!I$}}           %% I-I
\def\VminV{\hbox{$V\!\!-\!\!V$}}           %% V-V
\def\Xt{\hbox{$X\!\!-\!t$}}                %% X-t

\def\sun{\hbox{$\odot$}}                   %% Sun symbol
\def\earth{\hbox{$\oplus$}}                %% Earth symbol

\def\BminV{\hbox{$B\!\!-\!\!V$}}           %% B-V
\def\VminIk{\hbox{$(V\!\!-\!\!I)_K$}}      %% V-I_K
\def\Teff{\hbox{$T_{\rm eff}$}}            %% T_eff

\def\Bapp{\hbox{$B_{\rm app}$}}              %% apparent flux density
\def\Basp{\hbox{$B_{\rm app}^{\rm ASP}$}}    %% apparent flux density ASP
\def\Bbbso{\hbox{$B_{\rm app}^{\rm BBSO}$}}  %% idem BBSO
\def\Bkpno{\hbox{$B_{\rm app}^{\rm KPNO}$}}  %% idem KPNO

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% stacked math symbols
%% macro by Louis Strous, after char.mac Skumanich Soesterberg 
%% usage: \mathstacksym\newsymbol{upper_symbol}{lower_symbol}
%%                               {upper_height}{lower_depth}
\def\mathstacksym#1#2#3#4#5{\def#1{\mathrel{\hbox to 0pt{\lower 
    #5\hbox{#3}\hss} \raise #4\hbox{#2}}}}

\mathstacksym\lta{$<$}{$\sim$}{1.5pt}{3.5pt} % less than approximately
\mathstacksym\gta{$>$}{$\sim$}{1.5pt}{3.5pt} % greater than approximately
\mathstacksym\lrarrow{$\leftarrow$}{$\rightarrow$}{2pt}{1pt} % equilibrium
\mathstacksym\lessgreat{$>$}{$<$}{3pt}{3pt} %% less or greater

%%%%%%%%%%%%%%%%%%%%  END OF FILE RRMACROS.TEX  %%%%%%%%%%%%%%%%%%%%%%%%%%%


==> h3318aa <==
%% file: AAJOUR.BIB = journal strings, new AA & AoJ abbreviations
%% last: Oct 31 1995
%% baton: Rob Rutten, Sterrekundig Instituut Utrecht
%%     >> don't change this file - its baton is mine all the time <<

@STRING{acta = "Acta Astron."}
@STRING{actastsin = "Acta Astron.\ Sin."}
@STRING{actapsin = "Acta Astrophys.\ Sin."}
@STRING{advp = "Adv.\ Phys."}
@STRING{advsr = "Adv.\ Space Res."}
@STRING{amjp = "Am.\ J.\ Phys."}
@STRING{annap = "Ann.\ d'Astrophys."}
@STRING{annrev = "ARA\hbox{\rm \&}A"}
@STRING{araa = "ARA\hbox{\rm \&}A"}
@STRING{ao = "Appl.\ Opt."}
@STRING{appl = "Appl.\ Phys.\ Lett."}
@STRING{apb = "Appl.\ Phys.\ B"}
@STRING{afz = "Afz"}
@STRING{aa = "A\hbox{\rm \&}A"}
@STRING{aar = "A\hbox{\rm \&}AR"}
@STRING{aas = "A\hbox{\rm \&}AS"}
@STRING{agas = "Astron.\ Ges.\ Abstr.\ Ser."}
@STRING{aj = "AJ"}
@STRING{an = "Astron.\ Nachr."}
@STRING{azh = "AZh"}
@STRING{apj = "ApJ"}
@STRING{apjl = "ApJ"}
@STRING{apjss = "ApJS"}
@STRING{apss = "Ap\hbox{\rm \&}SS"}
@STRING{ap = "Astrophysics"}
@STRING{ajp = "Aust.\ J.\ Phys."}
@STRING{baas = "BAAS"}
@STRING{ban = "Bull.\ Astron.\ Inst.\ Neth."}
@STRING{bac = "Bull.\ Astron.\ Inst.\ Czech."}
@STRING{cjp = "Can.\ J.\ Phys."}
@STRING{cm = "Celest.\ Mech."}
@STRING{chinaa = "Chin.\ Astron."}
@STRING{cast = "Comments Astrophys."}
@STRING{fiz = "Fizika"}
@STRING{gafd = "Geophys.\ Astrophys.\ Fluid Dyn."}
@STRING{gj = "Geophys.\ J."}
@STRING{grl = "Geophys.\ Res.\ Lett."}
@STRING{geo = "Geophysics"}
@STRING{hd = "Hemel en Dampkring"}
@STRING{iauc = "IAU Circ."}
@STRING{iauib = "IAU Inf.\ Bull."}
@STRING{icarus = "Icarus"}
@STRING{jap = "J.\ Appl.\ Phys."}
@STRING{jaa = "JA\hbox{\rm \&}A"}
@STRING{jas = "J.\ Atmos.\ Sci."}
@STRING{jchemp = "J.\ Chem.\ Phys."}
@STRING{jcomp = "J.\ Comp.\ Phys."}
@STRING{jfm = "J.\ Fluid Mech."}
@STRING{jgr = "J.\ Geophys.\ Res."}
@STRING{jhast = "J.\ Hist.\ Astron."}
@STRING{jmolspec = "J.\ Mol.\ Spectrosc."}
@STRING{josa = "J.\ Opt.\ Soc.\ Am."}
@STRING{josaa = "J.\ Opt.\ Soc.\ Am.\ A"}
@STRING{josab = "J.\ Opt.\ Soc.\ Am.\ B"}
@STRING{jp = "J.\ Phys."}
@STRING{jpa = "J.\ Phys.\ A"}
@STRING{jpb = "J.\ Phys.\ B"}
@STRING{jpd = "J.\ Phys.\ D"}
@STRING{jpe = "J.\ Phys.\ E"}
@STRING{jpg = "J.\ Phys.\ G"}
@STRING{jpsj = "J.\ Phys.\ Soc.\ Japan"}
@STRING{jpp = "J.\ Plasma Phys."}
@STRING{jqsrt = "J.\ Quant.\ Spectrosc.\ Radiat.\ Transfer"}
@STRING{jrasc = "J.\ R.\ Astron.\ Soc.\ Can."}
@STRING{jetpl = "JETP Lett."}
@STRING{kfnt = "Kinematika Fiz.\ Nebesn.\ Tel"}
@STRING{msai = "Mem.\ Soc.\ Astron.\ Ital."}
@STRING{merc = "Mercury"}
@STRING{mag = "Mitt.\ Astron.\ Ges."}
@STRING{mn = "MNRAS"}
@STRING{mnras = "MNRAS"}
@STRING{mnassa = "Mon.\ Notes Astron.\ Soc.\ S.\ Afr."}
@STRING{nat = "Nat"}
@STRING{nature="Nat"}
@STRING{natwis = "Naturwissenschaften"}
@STRING{nattech = "Natuur en Techniek"}
@STRING{obs = "Observatory"}
@STRING{pfa = "Phys.\ Fluids A"}
@STRING{pfb = "Phys.\ Fluids B"}
@STRING{pla = "Phys.\ Lett.\ A"}
@STRING{plb = "Phys.\ Lett.\ B"}
@STRING{pra = "Phys.\ Rev.\ A"}
@STRING{prb = "Phys.\ Rev.\ B"}
@STRING{prc = "Phys.\ Rev.\ C"}
@STRING{prd = "Phys.\ Rev.\ D"}
@STRING{prl = "Phys.\ Rev.\ Lett."}
@STRING{ps = "Phys.\ Scr."}
@STRING{ptod = "Phys.\ Today"}
@STRING{pha = "Physica A"}
@STRING{phb = "Physica B"}
@STRING{phd = "Physica D"}
@STRING{pss = "Planet.\ Space Sci."}
@STRING{ppcf = "Plasma Phys.\ Controlled Fusion"}
@STRING{pasa = "Proc.\ Astron.\ Soc.\ Aust."}
@STRING{pi3e = "Proc.\ IEEE"}
@STRING{prsl = "Proc.\ R.\ Soc.\ London Ser.\ A"}
@STRING{posp = "Proceedings of SPIE"}
@STRING{pasj = "PASJ"}
@STRING{pasp = "PASP"}
@STRING{paspc = "PASPC"}
@STRING{qjras = "QJRAS"}
@STRING{ra = "Rev.\ Astron."}
@STRING{sciam = "Sci.\ Am."}
@STRING{sc = "Sci"}
@STRING{sky = "Sky Telesc."}
@STRING{sp = "Solar Phys."}
@STRING{sdb = "Soln.\ Dannye Byull."}
@STRING{sonne = "Sonne"}
@STRING{sa = "SvA"}
@STRING{sal = "SvA"}
@STRING{ssr = "Space Sci.\ Rev."}
@STRING{sf = "Spaceflight"}
@STRING{sterne = "Sterne"}
@STRING{sw = "Sterne Weltraum"}
@STRING{uao = "Upps.\ Astron.\ Obs.\ Rep."}
@STRING{va = "Vistas Astron."}
@STRING{zpa = "Z.\ Phys.\ A"}
@STRING{zpc = "Z.\ Phys.\ C"}
@STRING{zenit = "Zenit"}
@STRING{zetf = "Zh.\ Ehksp.\ Teor.\ Fiz."}
@STRING{ZsAp = "Zs.\ f.\ Ap."}
@STRING{ZsP = "Zs.\ f.\ Phys."}


==> h3318bib <==
@ARTICLE{Abia1988A&A...206..100A,
    author = {{Abia}, C. and {Rebolo}, R. and {Beckman}, J.\ E. and {Crivellari}, L.
        },
    title = {Abundances of light metals and NI in a sample of disc stars},
    journal = {\aap},
    year = 1988,
    month = nov,
    volume = 206,
    pages = {100--107},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988A%26A...206..100A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Abia1998MNRAS.293...89A,
    author = {{Abia}, C. and {Wallerstein}, G.},
    title = "Heavy-element abundances in seven SC stars and several related stars",
    journal = {\mnras},
    year = 1998,
    month = jan,
    volume = 293,
    pages = {89},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998MNRAS.293...89A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Achmad1991A&A...249..192A,
    author = {{Achmad}, L. and {de Jager}, C. and {Nieuwenhuijzen}, H.},
    title = {Atmospheric model parameters and shock wave field for the supergiant Alpha Carinae (F0Ib)},
    journal = {\aap},
    year = 1991,
    month = sep,
    volume = 249,
    pages = {192--198},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...249..192A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Adelman1990ApJ...348..712A,
    author = {{Adelman}, S.\ J. and {Gulliver}, A.\ F.},
    title = "An elemental abundance analysis of the superficially normal A star VEGA",
    journal = {\apj},
    year = 1990,
    month = jan,
    volume = 348,
    pages = {712--717},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJ...348..712A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Allard1992RMxAA..23..203A,
    author = {{Allard}, F. and {Scholz}, M. and {Wehrse}, R.},
    title = "Molecular opacities in M-star atmospheres.",
    journal = {Revista Mexicana de Astronomia y Astrofisica},
    year = 1992,
    month = mar,
    volume = 23,
    pages = {203--215},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992RMxAA..23..203A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Altas1987Ap&SS.134...85A,
    author = {{Altas}, L.},
    title = "Carbon, nitrogen, and oxygen abundances in Procyon, sun, and Arcturus",
    journal = {\apss},
    year = 1987,
    month = jun,
    volume = 134,
    pages = {85--94},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987Ap%26SS.134...85A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Anders1989GeCoA..53..197A,
    author = {{Anders}, E. and {Grevesse}, N.},
    title = "{Abundances of the elements - Meteoritic and solar}",
    journal = {\gca},
    year = 1989,
    month = jan,
    volume = 53,
    pages = {197--214},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989GeCoA..53..197A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Aoki1997A&A...328..175A,
    author = {{Aoki}, W. and {Tsuji}, T.},
    title = "High resolution infrared spectroscopy of CN and NH lines:  nitrogen abundance in oxygen-rich giants through K to late M",
    journal = {\aap},
    year = 1997,
    month = dec,
    volume = 328,
    pages = {175--186},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...328..175A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Aringer1999A&A...342..799A,
    author = {{Aringer}, B. and {H{\"o}fner}, S. and {Wiedemann}, G. and {Hron}, J. and 
        {J{\o}rgensen}, U.\ G. and {K{\"a}ufl}, H.\ U. and {Windsteig}, W.
        },
    title = "SiO rotation-vibration bands in cool giants II. The behaviour of SiO bands in AGB stars",
    journal = {\aap},
    year = 1999,
    month = feb,
    volume = 342,
    pages = {799--808},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...342..799A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Asplund2000A&A...359..729A,
    author = {{Asplund}, M. and {Nordlund}, {\AA}. and {Trampedach}, R. and 
        {Allende Prieto}, C. and {Stein}, R.\ F.},
    title = {Line formation in solar granulation. I. Fe line shapes, shifts and asymmetries},
    journal = {\aap},
    year = 2000,
    month = jul,
    volume = 359,
    pages = {729--742},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...359..729A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ayres1982ApJ...263..791A,
    author = {{Ayres}, T.~R. and {Simon}, T. and {Linsky}, J.~L.},
    title = "{Evolution of chromospheres and coronae in solar mass stars - A far-ultraviolet and soft X-ray comparison of Arcturus /K2 III/ and Alpha Centauri A /G2 V/}",
    journal = {\apj},
    year = 1982,
    month = dec,
    volume = 263,
    pages = {791--802},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...263..791A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Balona1984MNRAS.211..973B,
    author = {{Balona}, L.\ A.},
    title = "Calibration of effective temperature, bolometric correction and mass for early-type stars using Stroemgren photometric indices",
    journal = {\mnras},
    year = 1984,
    month = dec,
    volume = 211,
    pages = {973--979},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984MNRAS.211..973B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Barklem2000A&A...355L...5B,
    author = {{Barklem}, P.\ S. and {Piskunov}, N. and {O'Mara}, B.\ J.},
    title = {Self broadening of hydrogen lines: initial results},
    journal = {\aap},
    year = 2000,
    month = mar,
    volume = 355,
    pages = {L5--L8},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...355L...5B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Barnes1976MNRAS.174..489B,
    author = {{Barnes}, T.\ G. and {Evans}, D.\ S.},
    title = "Stellar angular diameters and visual surface brightness. I. Late spectral types.",
    journal = {\mnras},
    year = 1976,
    month = mar,
    volume = 174,
    pages = {489--502},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976MNRAS.174..489B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Barnes1976MNRAS.174..503B,
    author = {{Barnes}, T.\ G. and {Evans}, D.\ S. and {Parsons}, S.\ B.},
    title = "Stellar angular diameters and visual surface brightness. II. Early and intermediate spectral types.",
    journal = {\mnras},
    year = 1976,
    month = mar,
    volume = 174,
    pages = {503--512},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976MNRAS.174..503B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Basri1979ApJ...234.1023B,
    author = {{Basri}, G.\ S. and {Linsky}, J.\ L.},
    title = "Outer atmospheres of cool stars. II - MG II flux profiles and chromospheric radiative loss rates",
    journal = {\apj},
    year = 1979,
    month = dec,
    volume = 234,
    pages = {1023--1035},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...234.1023B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Becker1981ApJS...45..475B,
    author = {{Becker}, S.~A.},
    title = "{The evolution of intermediate-mass stars from the zero-age main sequence to the base of the asymptotic giant branch as a function of mass and composition}",
    journal = {\apjs},
    year = 1981,
    month = mar,
    volume = 45,
    pages = {475--505},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJS...45..475B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bell1981ApJ...248.1031B,
    author = {{Bell}, R.\ A. and {Dreiling}, L.\ A.},
    title = "The chemical composition, gravity, and temperature of Sirius",
    journal = {\apj},
    year = 1981,
    month = sep,
    volume = 248,
    pages = {1031--1042},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...248.1031B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bell1985MNRAS.212..497B,
    author = {{Bell}, R.\ A. and {Edvardsson}, B. and {Gustafsson}, B.},
    title = "The surface gravity of Arcturus from MgH lines, strong metal lines and the ionization equilibrium of iron",
    journal = {\mnras},
    year = 1985,
    month = feb,
    volume = 212,
    pages = {497--515},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985MNRAS.212..497B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bell1989MNRAS.236..653B,
    author = {{Bell}, R.\ A. and {Gustafsson}, B.},
    title = "The effective temperatures and colours of G and K stars",
    journal = {\mnras},
    year = 1989,
    month = feb,
    volume = 236,
    pages = {653--707},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989MNRAS.236..653B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bessell1984PASP...96..247B,
    author = {{Bessell}, M.~S. and {Wood}, P.~R.},
    title = "{A note on bolometric corrections for late-type stars and long-period variables}",
    journal = {\pasp},
    year = 1984,
    month = mar,
    volume = 96,
    pages = {247--249},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984PASP...96..247B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bessell1998A&A...333..231B,
    author = {{Bessell}, M.~S. and {Castelli}, F. and {Plez}, B.},
    title = "{Model atmospheres broad-band colors, bolometric corrections  and temperature calibrations for O - M stars}",
    journal = {\aap},
    year = 1998,
    month = may,
    volume = 333,
    pages = {231--250},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...333..231B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1977MNRAS.180..177B,
    author = {{Blackwell}, D.\ E. and {Shallis}, M.\ J.},
    title = {Stellar angular diameters from infrared photometry - Application to Arcturus and other stars; with effective temperatures},
    journal = {\mnras},
    year = 1977,
    month = jul,
    volume = 180,
    pages = {177--191},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1977MNRAS.180..177B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1980A&A....82..249B,
    author = {{Blackwell}, D.\ E. and {Petford}, A.\ D. and {Shallis}, M.\ J.
        },
    title = {Use of the infra-red flux method for determining stellar effective temperatures and angular diameters - The stellar temperature scale},
    journal = {\aap},
    year = 1980,
    month = feb,
    volume = 82,
    pages = {249--252},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980A%26A....82..249B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1990A&A...232..396B,
    author = {{Blackwell}, D.\ E. and {Petford}, A.\ D. and {Haddock}, D.\ J. and 
        {Arribas}, S. and {Selby}, M.\ J.},
    title = {Determination of temperatures and angular diameters of 114 F-M stars using the infrared flux method (IRFM)},
    journal = {\aap},
    year = 1990,
    month = jun,
    volume = 232,
    pages = {396--410},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26A...232..396B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}
@ARTICLE{Blackwell1991A&A...245..567B,
    author = {{Blackwell}, D.\ E. and {Lynas-Gray}, A.\ E. and {Petford}, A.\ D.
        },
    title = "Effect of improved H$^-$ opacity on the infrared flux method temperature scale and derived angular diameters - Use of a self-consistent calibration", 
    journal = {\aap},
    year = 1991,
    month = may,
    volume = 245,
    pages = {567--574},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...245..567B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1998A&AS..129..505B,
    author = {{Blackwell}, D.\ E. and {Lynas-Gray}, A.\ E.},
    title = "Determination of the temperatures of selected ISO flux calibration stars using the Infrared Flux Method",
    journal = {\aaps},
    year = 1998,
    month = may,
    volume = 129,
    pages = {505--515},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26AS..129..505B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{BohmVitense1981ARA&A..19..295B,
    author = {{B\"{o}hm-Vitense}, E.},
    title = "{The effective temperature scale}",
    journal = {\araa},
    year = 1981,
    volume = 19,
    pages = {295--317},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ARA%26A..19..295B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Bonnell1982MNRAS.201..253B,
    author = {{Bonnell}, J. and {Bell}, R.\ A.},
    title = "Carbon and nitrogen abundances in Population I G and K giant stars from DDO photometry",
    journal = {\mnras},
    year = 1982,
    month = oct,
    volume = 201,
    pages = {253--263},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.201..253B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bonnell1993MNRAS.264..319B,
    author = {{Bonnell}, J.~T. and {Bell}, R.~A.},
    title = "{The Gravities of K Giant Stars Determined from OI and OH Features}",
    journal = {\mnras},
    year = 1993,
    month = sep,
    volume = 264,
    pages = {319},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993MNRAS.264..319B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Boyarchuk1983Ap.....18..228B,
    author = {{Boyarchuk}, A.\ A. and {Lyubimkov}, L.\ S.},
    title = {The Atmosphere of Canopus - Part One - Model of the Atmosphere and Distribution of the Microturbulence},
    journal = {Astrophysics},
    year = 1983,
    volume = 18,
    pages = {228},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983Ap.....18..228B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Brown1974MNRAS.167..121B,
    author = {{Brown}, R.\ H. and {Davis}, J. and {Allen}, L.\ R.},
    title = {The angular diameters of 32 stars.},
    journal = {\mnras},
    year = 1974,
    month = apr,
    volume = 167,
    pages = {121--136},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974MNRAS.167..121B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Brown1983ApJ...265L..93B,
    author = {{Brown}, J.\ A. and {Tomkin}, J. and {Lambert}, D.\ L.},
    title = {Evidence of non-LTE in photospheric lines of G and K giants},
    journal = {\apjl},
    year = 1983,
    month = feb,
    volume = 265,
    pages = {L93--L97},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983ApJ...265L..93B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Brown1989ApJS...71..293B,
    author = {{Brown}, J.\ A. and {Sneden}, C. and {Lambert}, D.\ L. and {Dutchover}, E.\ J.
        },
    title = "A search for lithium-rich giant stars",
    journal = {\apjs},
    year = 1989,
    month = oct,
    volume = 71,
    pages = {293--322},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989ApJS...71..293B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Burnashev1983IzKry..67...13B,
    author = {{Burnashev}, V.\ I.},
    title = "A determination of the effective temperatures, accelerations of gravity, and metallicity parameters of late-type stars from data on energy distribution in their spectra",
    journal = {Izvestiya Ordena Trudovogo Krasnogo Znameni Krymskoj Astrofizicheskoj Observatorii},
    year = 1983,
    volume = 67,
    pages = {13--33},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983IzKry..67...13B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@INPROCEEDINGS{Cami1997fiso.work..159C,                                       
        AUTHOR  = {{Cami}, J. and {Justtanont}, K. and {de Jong}, T. and {Feuchtgruber}, H. and 
        {Tielens}, A.\ G.\ G.\ M. and {Yamamura}, I. and {Waters}, L.\ B.\ F.\ M.
        }, 
        TITLE   = "CO$_2$ Emission in O-Rich AGB Stars",
        BOOKTITLE = {The first ISO workshop on Analytical Spectroscopy},
        YEAR    = 1997,
        PAGES   = {159},
      EDITOR    = {{Heras}, A.\ M. and {Leech}, K. and {Trams}, N.\ R. and {Perry}, M.},
        ADDRESS = "ESA SP-419"}


@ARTICLE{Castelli1994A&A...281..817C,
    author = {{Castelli}, F. and {Kurucz}, R.~L.},
    title = "{Model atmospheres for VEGA}",
    journal = {\aap},
    year = 1994,
    month = jan,
    volume = 281,
    pages = {817--832},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...281..817C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cayrel1985A&A...146..249C,
    author = {{Cayrel}, R. and {Cayrel de Strobel}, G. and {Campbell}, B.},
    title = "Steps towards the abundance scale. I - The abundance of heavy elements in the Hyades cluster",
    journal = {\aap},
    year = 1985,
    month = may,
    volume = 146,
    pages = {249--259},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985A%26A...146..249C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cayrel1992A&AS...95..273C,
    author = {{Cayrel de Strobel}, G. and {Hauck}, B. and {Francois}, P. and 
        {Thevenin}, F. and {Friel}, E. and {Mermilliod}, M. and {Borde}, S.
        },
    title = "{A catalogue of Fe/H determinations - 1991 edition}",
    journal = {\aaps},
    year = 1992,
    month = oct,
    volume = 95,
    pages = {273--336},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26AS...95..273C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Charbonnel1994A&A...282..811C,
    author = {{Charbonnel}, C.},
    title = "Clues for non-standard mixing on the red giant branch from C-12/C-13 and C-12/N-14 ratios in evolved stars",
    journal = {\aap},
    year = 1994,
    month = feb,
    volume = 282,
    pages = {811--820},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...282..811C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Charbonnel1995ApJ...453L..41C,
    author = {{Charbonnel}, C.},
    title = "A Consistent Explanation for 12C/ 13C, 7Li and 3He Anomalies in Red Giant Stars",
    journal = {\apjl},
    year = 1995,
    month = nov,
    volume = 453,
    pages = {L41},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995ApJ...453L..41C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Charbonnel1998A&A...332..204C,
    author = {{Charbonnel}, C. and {Brown}, J.\ A. and {Wallerstein}, G.},
    title = "Mixing processes during the evolution of red giants with moderate metal deficiencies: the role of molecular-weight barriers",
    journal = {\aap},
    year = 1998,
    month = apr,
    volume = 332,
    pages = {204--214},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...332..204C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Chmielewski1992A&A...263..219C,
    author = {{Chmielewski}, Y. and {Friel}, E. and {Cayrel de Strobel}, G. and 
        {Bentolila}, C.},
    title = {The 1992 detailed analyses of Alpha Centauri A and Alpha Centauri B},
    journal = {\aap},
    year = 1992,
    month = sep,
    volume = 263,
    pages = {219--231},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...263..219C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ciardi2001ApJ...559.1147C,
    author = {{Ciardi}, D.~R. and {van Belle}, G.~T. and {Akeson}, R.~L. and 
        {Thompson}, R.~R. and {Lada}, E.~A. and {Howell}, S.~B.},
    title = "{On the Near-Infrared Size of Vega}",
    journal = {\apj},
    year = 2001,
    month = oct,
    volume = 559,
    pages = {1147--1154},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...559.1147C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Claret1995A&AS..114..549C,
    author = {{Claret}, A. and {Gimenez}, A.},
    title = "Stellar models for a wide range of initial chemical compositions until helium burning. II. From X=0.63 to X=0.80, for Z=0.01.",
    journal = {\aaps},
    year = 1995,
    month = dec,
    volume = 114,
    pages = {549},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26AS..114..549C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Clegg1979ApJ...234..188C,
    author = {{Clegg}, R.\ E.\ S. and {Lambert}, D.\ L. and {Bell}, R.\ A.
        },
    title = "Isotopes of titanium in cool stars",
    journal = {\apj},
    year = 1979,
    month = nov,
    volume = 234,
    pages = {188--199},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...234..188C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Code1976ApJ...203..417C,
    author = {{Code}, A.\ D. and {Bless}, R.\ C. and {Davis}, J. and {Brown}, R.\ H.
        },
    title = {Empirical effective temperatures and bolometric corrections for early-type stars},
    journal = {\apj},
    year = 1976,
    month = jan,
    volume = 203,
    pages = {417--434},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...203..417C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1992AJ....104.1650C,
    author = {{Cohen}, M. and {Walker}, R.\ G. and {Barlow}, M.\ J. and {Deacon}, J.\ R.
        },
    title = "Spectral irradiance calibration in the infrared. I - Ground-based and IRAS broadband calibrations",
    journal = {\aj},
    year = 1992,
    month = oct,
    volume = 104,
    pages = {1650--1657},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....104.1650C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1992AJ....104.2030C,
    author = {{Cohen}, M. and {Walker}, R.\ G. and {Witteborn}, F.\ C.},
    title = {Spectral irradiance calibration in the infrared. II - Alpha Tau
                  and the recalibration of the IRAS low resolution
                  spectrometer}, 
    journal = {\aj},
    year = 1992,
    month = nov,
    volume = 104,
    pages = {2030--2044},
    url =   {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....104.2030C&db_key=AST}, 
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1995AJ....110..275C,
    author = {{Cohen}, M. and {Witteborn}, F.\ C. and {Walker}, R.\ G. and 
        {Bregman}, J.\ D. and {Wooden}, D.\ H.},
    title = {Spectral Irradiance Calibration in the Infrared.IV. 1.2-35 micron spectra of six standard stars},
    journal = {\aj},
    year = 1995,
    month = jul,
    volume = 110,
    pages = {275},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995AJ....110..275C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1996AJ....112..241C,
    author = {{Cohen}, M. and {Witteborn}, F.\ C. and {Bregman}, J.\ D. and 
        {Wooden}, D.\ H. and {Salama}, A. and {Metcalfe}, L.},
    title = {Spectral Irradiance Calibration in the Infrared. VI. 3-35 micron Spectra of Three Southern Standard Stars},
    journal = {\aj},
    year = 1996,
    month = jul,
    volume = 112,
    pages = {241},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996AJ....112..241C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1996AJ....112.2274C,
    author = {{Cohen}, M. and {Witteborn}, F.\ C. and {Carbon}, D.\ F. and 
        {Davies}, J.\ K. and {Wooden}, D.\ H. and {Bregman}, J.\ D.},
    title = {Spectral Irradiance Calibration in the Infrared.VII.New Composite Spectra, Comparison with Model Atmospheres, and Far-Infrared Extrapolations},
    journal = {\aj},
    year = 1996,
    month = nov,
    volume = 112,
    pages = {2274},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996AJ....112.2274C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1999AJ....117.1864C,
    author = {{Cohen}, M. and {Walker}, R.\ G. and {Carter}, B. and {Hammersley}, P. and 
        {Kidger}, M. and {Noguchi}, K.},
    title = "Spectral Irradiance Calibration in the Infrared. X. A Self-Consistent Radiometric All-Sky Network of Absolutely Calibrated Stellar Spectra",
    journal = {\aj},
    year = 1999,
    month = apr,
    volume = 117,
    pages = {1864--1889},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999AJ....117.1864C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cornide1992AJ....103.1374C,
    author = {{Cornide}, M. and {Fernandez-Figueroa}, M.\ J. and {de Castro}, E. and 
        {Armentia}, J.\ A. and {Reglero}, V.},
    title = "Stellar activity in barium stars. I - Analysis of H and K CA II lines in ten barium stars",
    journal = {\aj},
    year = 1992,
    month = apr,
    volume = 103,
    pages = {1374--1380},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....103.1374C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cousins1972MNSSA..31...69C,
    author = {{Cousins}, A.~W.~J.},
    title = "{UBV photometry of some very bright stars}",
    journal = {Monthly Notes of the Astronomical Society of South Africa},
    year = 1972,
    volume = 31,
    pages = {69},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1972MNSSA..31...69C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Currie1974ApJ...187..131C,
    author = {{Currie}, D.~G. and {Knapp}, S.~L. and {Liewer}, K.~M.},
    title = "{Four stellar-diameter measurements by a new technique : amplitude interferometry.}",
    journal = {\apj},
    year = 1974,
    month = jan,
    volume = 187,
    pages = {131--134},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974ApJ...187..131C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Davis1998IAUS..189...31D,
    author = {{Davis}, J.},
    title = "{Stellar angular diameter measurements by interferometry}",
    booktitle = {IAU Symp. 189: Fundamental Stellar Properties},
    year = 1998,
    volume = 189,
    pages = {31},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998IAUS..189...31D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Dearborn1976ApJ...203..455D,
    author = {{Dearborn}, D.~S.~P. and {Eggleton}, P.~P. and {Schramm}, D.~N.
        },
    title = "{12C/13C ratios in stars ascending the giant branch the first time.}",
    journal = {\apj},
    year = 1976,
    month = jan,
    volume = 203,
    pages = {455--462},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...203..455D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dearborn1975ApJ...200..675D,
    author = {{Dearborn}, D.\ S.\ P. and {Lambert}, D.\ L. and {Tomkin}, J.
        },
    title = "The C-12/C-13 ratio in stellar atmospheres. V - Twelve K giants and subgiants",
    journal = {\apj},
    year = 1975,
    month = sep,
    volume = 200,
    pages = {675--681},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975ApJ...200..675D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Decat2000A&A...355.1015D,
    author = {{De Cat}, P. and {Aerts}, C. and {De Ridder}, J. and {Kolenberg},
                  K. and  {Meeus}, G. and {Decin}, L.},
    title = {A study of bright southern slowly pulsating B
                  stars. I. Determination of the orbital parameters and of the
                  main frequency  of the spectroscopic binaries}, 
    journal = {\aap},
    year = 2000,
    month = mar,
    volume = 355,
    pages = {1015--1030},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...355.1015D&db_key=AST}, 
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Decin1997fiso.work..185D,
    author = {{Decin}, L. and {Cohen}, M. and {Eriksson}, K. and {Gustafsson}, B. and 
        {Huygen}, E. and {Morris}, P. and {Plez}, B. and {Sauval}, J. and 
        {Vandenbussche}, B. and {Waelkens}, C.},
    title = {Comparison Bertween ISO-SWS Observations and Synthetic Spectra of K Giants and M Giants: $\alpha$ Boo and {\&} $\beta$ Peg},
    booktitle = {The first ISO workshop on Analytical Spectroscopy},
    year = 1997,
    pages = {185},
      EDITOR    = {{Heras}, A.\ M. and {Leech}, K. and {Trams}, N.\ R. and {Perry}, M.},
        ADDRESS = "ESA SP-419"}




@PHDTHESIS{Decinthesis,
    author = {{Decin}, L.},
    title = {Synthetic spectra of cool stars observed with the Short-Wavelength Spectrometer: improving the models and the calibration of the instrument},
    school = {University of Leuven},
    year = 2000,
}

@ARTICLE{Decin2000A&A...364..137D,
    author = {{Decin}, L. and {Waelkens}, C. and {Eriksson}, K. and {Gustafsson}, B. and 
        {Plez}, B. and {Sauval}, A.\ J. and {Van Assche}, W. and
                  {Vandenbussche}, B. 
        }, 
    title = "ISO-SWS calibration and the accurate modelling  of
                  cool-star atmospheres. I.\ Method", 
    journal = {\aap},
    year = 2000,
    month = dec,
    volume = 364,
    pages = {137--156},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...364..137D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Decin2000b,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and  
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: II.\ Results", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in press},
        PAGES   = {(Paper~II)}
}

@ARTICLE{Decin2000c,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and 
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: III.\ A0 to G2 stars", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in press},
        PAGES   = {(Paper~III)}
}

@ARTICLE{Decin2000d,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and 
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: IV.\ G9 to M2 stars", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in press},
        PAGES   = {(Paper~IV)}
}

@ARTICLE{Decin2000e,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and 
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: V.\ ", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in prep.},
        PAGES   = {}
}



@ARTICLE{deGraauw1996A&A...315L..49D,
    author = {{de Graauw}, T. and {Haser}, L.\ N. and {Beintema}, D.\ A. and 
        {Roelfsema}, P.\ R. and {van Agthoven}, H. and {Barl}, L. and 
        {Bauer}, O.\ H. and {Bekenkamp}, H.\ E.\ G. and {Boonstra}, A.\ -. and 
        {Boxhoorn}, D.\ R. and {Cote}, J. and {de Groene}, P. and {van Dijkhuizen}, C. and 
        {Drapatz}, S. and {Evers}, J. and {Feuchtgruber}, H. and {Frericks}, M. and 
        {Genzel}, R. and {Haerendel}, G. and {Heras}, A.\ M. and {van der Hucht}, K.\ A. and 
        {van der Hulst}, T. and {Huygen}, R. and {Jacobs}, H. and {Jakob}, G. and 
        {Kamperman}, T. and {Katterloher}, R.\ O. and {Kester}, D.\ J.\ M. and 
        {Kunze}, D. and {Kussendrager}, D. and {Lahuis}, F. and {Lamers}, H.\ J.\ G.\ L.\ M. and 
        {Leech}, K. and {van der Lei}, S. and {van der Linden}, R. and 
        {Luinge}, W. and {Lutz}, D. and {Melzner}, F. and {Morris}, P.\ W. and 
        {van Nguyen}, D. and {Ploeger}, G. and {Price}, S. and {Salama}, A. and 
        {Schaeidt}, S.\ G. and {Sijm}, N. and {Smoorenburg}, C. and 
        {Spakman}, J. and {Spoon}, H. and {Steinmayer}, M. and {Stoecker}, J. and 
        {Valentijn}, E.\ A. and {Vandenbussche}, B. and {Visser}, H. and 
        {Waelkens}, C. and {Waters}, L.\ B.\ F.\ M. and {Wensink}, J. and 
        {Wesselius}, P.\ R. and {Wiezorrek}, E. and {Wieprecht}, E. and 
        {Wijnbergen}, J.\ J. and {Wildeman}, K.\ J. and {Young}, E.},
    title = "Observing with the ISO Short-Wavelength Spectrometer.",
    journal = {\aap},
    year = 1996,
    month = nov,
    volume = 315,
    pages = {L49--L54},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...315L..49D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{deJong1999,                                       
        AUTHOR  = {{de Jong}, T.}, 
        TITLE   = "",
        BOOKTITLE = "Abstracts of the 2nd Austrian ISO
Workshop. Atmospheres of M, S and C Giants.",
        YEAR    = 1999,
        PAGES   = "53",
      EDITOR    = {{Hron}, J.  and {H{\"{o}}fner}, S.},
        ADDRESS = ""}



@ARTICLE{Demarque1986ApJ...300..773D,
    author = {{Demarque}, P. and {Guenther}, D.\ B. and {van Altena}, W.\ F.
        },
    title = {The case of Alpha Centauri - Mass, age and p-mode oscillation spectrum},
    journal = {\apj},
    year = 1986,
    month = jan,
    volume = 300,
    pages = {773--778},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986ApJ...300..773D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Desikachary1982MNRAS.201..707D,
    author = {{Desikachary}, K. and {Hearnshaw}, J.\ B.},
    title = {The spectrum of Canopus. II - Analysis and composition},
    journal = {\mnras},
    year = 1982,
    month = nov,
    volume = 201,
    pages = {707--721},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.201..707D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{DiBenedetto1987A&A...188..114D,
    author = {{di Benedetto}, G.\ P. and {Rabbia}, Y.},
    title = {Accurate angular diameters and effective temperatures for eleven giants cooler than K0 by Michelson interferometry},
    journal = {\aap},
    year = 1987,
    month = dec,
    volume = 188,
    pages = {114--124},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987A%26A...188..114D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{DiBenedetto1993A&A...270..315D,
    author = {{di Benedetto}, G.~P.},
    title = "{Empirical effective temperatures and angular diameters of stars cooler than the sun}",
    journal = {\aap},
    year = 1993,
    month = mar,
    volume = 270,
    pages = {315--334},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...270..315D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{DiBenedetto1998A&A...339..858D,
    author = {{di Benedetto}, G.\ P.},
    title = "Towards a fundamental calibration of stellar parameters  of A, F, G, K dwarfs and giants",
    journal = {\aap},
    year = 1998,
    month = nov,
    volume = 339,
    pages = {858--871},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...339..858D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dreiling1980ApJ...241..736D,
    author = {{Dreiling}, L.\ A. and {Bell}, R.\ A.},
    title = "The chemical composition, gravity, and temperature of VEGA",
    journal = {\apj},
    year = 1980,
    month = oct,
    volume = 241,
    pages = {736--758},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJ...241..736D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Drira1997A&A...319..720D,
    author = {{Drira}, I. and {Hure}, J.\ M. and {Spielfiedel}, A. and {Feautrier}, N. and 
        {Roueff}, E.},
    title = "Infrared transitions probabilities and radiative opacity of SiO.",
    journal = {\aap},
    year = 1997,
    month = mar,
    volume = 319,
    pages = {720--724},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...319..720D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dyck1974ApJ...189...89D,
    author = {{Dyck}, H.\ M. and {Lockwood}, G.\ W. and {Capps}, R.\ W.},
    title = "Infrared fluxes spectral types and temperatures for very cool stars.",
    journal = {\apj},
    year = 1974,
    month = apr,
    volume = 189,
    pages = {89--100},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974ApJ...189...89D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dyck1998AJ....116..981D,
    author = {{Dyck}, H.\ M. and {van Belle}, G.\ T. and {Thompson}, R.\ R.
        },
    title = "Radii and Effective Temperatures for K and M Giants and Supergiants. II.",
    journal = {\aj},
    year = 1998,
    month = aug,
    volume = 116,
    pages = {981--986},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998AJ....116..981D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Edvardsson1988A&A...190..148E,
    author = {{Edvardsson}, B.},
    title = {Spectroscopic surface gravities and chemical compositions for 8 nearby single sub-giants},
    journal = {\aap},
    year = 1988,
    month = jan,
    volume = 190,
    pages = {148--166},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988A%26A...190..148E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Eggen1973PASP...85..379E,
    author = {{Eggen}, O.\ J.},
    title = "Luminosity and velocity distribution of high-luminosity stars near the sun. II. The young disk giants",
    journal = {\pasp},
    year = 1973,
    month = aug,
    volume = 85,
    pages = {379--395},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1973PASP...85..379E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{ElEid1994A&A...285..915E,
    author = {{El Eid}, M.\ F.},
    title = {CNO isotopes in red giants: theory versus observations},
    journal = {\aap},
    year = 1994,
    month = may,
    volume = 285,
    pages = {915--928},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...285..915E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Engelke1992AJ....104.1248E,
    author = {{Engelke}, C.\ W.},
    title = {Analytic approximations to the 2-60 microns infrared continua for standard calibration stars - With application to the calibration of spectroscopy and photometry, and the determination of effective temperature and angular size from IR measurements},
    journal = {\aj},
    year = 1992,
    month = sep,
    volume = 104,
    pages = {1248--1259},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....104.1248E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{England1980MNRAS.191...23E,
    author = {{England}, M.\ N.},
    title = {A spectroscopic analysis of the Alpha Centauri system},
    journal = {\mnras},
    year = 1980,
    month = apr,
    volume = 191,
    pages = {23--35},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980MNRAS.191...23E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Fagotto1994A&AS..105...29F,
    author = {{Fagotto}, F. and {Bressan}, A. and {Bertelli}, G. and {Chiosi}, C.
        },
    title = "{Evolutionary sequences of stellar models with new radiative opacities. IV. Z=0.004 and Z=0.008}",
    journal = {\aaps},
    year = 1994,
    month = may,
    volume = 105,
    pages = {29--38},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26AS..105...29F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Farmer1989QB551.F37......,
    author = {{Farmer}, C.\ B. and {Norton}, R.\ H.},
    title = {A High-Resolution Atlas of the Infrared Spectrum of the Sun and
                  Earth Atmosphere from Space.  Volume I. The Sun}, 
    publisher = {Washington, D.C.\ : NASA, Scientific and Technical Information Division},  
    year = 1989,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989QB551.F37......&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Faucherre1983A&A...120..263F,
    author = {{Faucherre}, M. and {Bonneau}, D. and {Koechlin}, L. and {Vakili}, F.
        },
    title = "Stellar interferometry - Diameters and effective temperatures of five giant stars",
    journal = {\aap},
    year = 1983,
    month = apr,
    volume = 120,
    pages = {263--268},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983A%26A...120..263F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Fernandez-Villacanas1990AJ.....99.1961F,
    author = {{Fern\'{a}ndez-Villaca\~{n}as}, J.\ L. and {Rego}, M. and {Cornide}, M.
        },
    title = "Barium and iron abundances in red giants",
    journal = {\aj},
    year = 1990,
    month = jun,
    volume = 99,
    pages = {1961--1970},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990AJ.....99.1961F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Feuchtgruber1998,
        AUTHOR  = "{Feuchtgruber}, H.",
        TITLE   = {Status of AOT01 AOT band order ratios
                    and related data}, 
      PUBLISHER = {ISO-SWS online documentation},
        YEAR    = 1998}

@ARTICLE{Flannery1978ApJ...221..175F,
    author = {{Flannery}, B.\ P. and {Ayres}, T.\ R.},
    title = {Evolution of the Alpha Centauri system},
    journal = {\apj},
    year = 1978,
    month = apr,
    volume = 221,
    pages = {175--185},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...221..175F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Flower1996ApJ...469..355F,
    author = {{Flower}, P.\ J.},
    title = "Transformations from Theoretical Hertzsprung-Russell Diagrams to Color-Magnitude Diagrams: Effective Temperatures, B-V Colors, and Bolometric Corrections",
    journal = {\apj},
    year = 1996,
    month = sep,
    volume = 469,
    pages = {355},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996ApJ...469..355F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Flynn1991A&A...250..400F,
    author = {{Flynn}, C. and {Mermilliod}, J.\ -.},
    title = "On the DDO absolute magnitudes of K giants",
    journal = {\aap},
    year = 1991,
    month = oct,
    volume = 250,
    pages = {400--406},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...250..400F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Fracassini1988BICDS..35..121F,
    author = {{Fracassini}, M. and {Pasinetti-Fracassini}, L.\ E. and {Pastori}, L. and 
        {Pironi}, R.},
    title = {Catalogue of Apparent Diameters and Absolute Radii of Stars},
    journal = {Bulletin d'Information du Centre de Donnees Stellaires},
    year = 1988,
    month = dec,
    volume = 35,
    pages = {121},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988BICDS..35..121F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Frisk1982MNRAS.199..471F,
    author = {{Frisk}, U. and {Nordh}, H.\ L. and {Olofsson}, S.\ G. and {Bell}, R.\ A. and 
        {Gustafsson}, B.},
    title = "The temperature of Arcturus",
    journal = {\mnras},
    year = 1982,
    month = may,
    volume = 199,
    pages = {471--481},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.199..471F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@BOOK{Fuhr1988atps.book.....F, 
    author = {{Fuhr}, J.\ R. and {Martin}, G.\ A. and {Wiese}, W.\ L.},
    title = {Atomic transition probabilities. Scandium through Manganese},
    publisher = {New York: American Institute of Physics (AIP) and American Chemical Society}, 
    year = 1988,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988atps.book.....F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@BOOK{Fuhr1988atpi.book.....F,
    author = {{Fuhr}, J.\ R. and {Martin}, G.\ A. and {Wiese}, W.\ L.},
    title = {Atomic transition probabilities. Iron through Nickel},
    publisher = {New York: American Institute of Physics (AIP) and American Chemical Society},
    year = 1988,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988atpi.book.....F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Furenlid1990ApJ...350..827F,
    author = {{Furenlid}, I. and {Meylan}, T.},
    title = {An abundance analysis of Alpha Centauri A},
    journal = {\apj},
    year = 1990,
    month = feb,
    volume = 350,
    pages = {827--838},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJ...350..827F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Johnson1966ARA&A...4..193J,
    author = {{Johnson}, H.~L.},
    title = "{Astronomical Measurements in the Infrared}",
    journal = {\araa},
    year = 1966,
    volume = 4,
    pages = {193},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1966ARA%26A...4..193J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Judge1986MNRAS.221..119J,
    author = {{Judge}, P.\ G.},
    title = "Constraints on the outer atmospheric structure of late-type giant stars with IUE - Methods and application to Arcturus (Alpha Boo K2III)",
    journal = {\mnras},
    year = 1986,
    month = jul,
    volume = 221,
    pages = {119--153},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986MNRAS.221..119J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Judge1991ApJ...371..357J,
    author = {{Judge}, P.\ G. and {Stencel}, R.\ E.},
    title = "Evolution of the chromospheres and winds of low- and intermediate-mass giant stars",
    journal = {\apj},
    year = 1991,
    month = apr,
    volume = 371,
    pages = {357--379},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991ApJ...371..357J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gadun1994AN....315..413G,
    author = {{Gadun}, A.\ S.},
    title = {Iron abundance and microturbulence in Arcturus, Canopus, alpha CEN A, and Sun from FeI and FeII lines},
    journal = {Astronomische Nachrichten},
    year = 1994,
    month = dec,
    volume = 315,
    pages = {413--418},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994AN....315..413G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gardiner1999A&A...347..876G,
    author = {{Gardiner}, R.~B. and {Kupka}, F. and {Smalley}, B.},
    title = "{Testing convection theories using Balmer line profiles of A, F, and G stars}",
    journal = {\aap},
    year = 1999,
    month = jul,
    volume = 347,
    pages = {876--890},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...347..876G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Geller1992,
    author = {{Geller}, M.},
    title = {A High-Resolution Atlas of the Infrared Spectrum of the Sun and
                  Earth Atmosphere from Space. Volume III. Key to Identification
                  of Solar Features},
    publisher = {Washington, D.C.\ : NASA, Scientific and Technical Information                  Division},   
    year = 1992,
    url = {},
}

@ARTICLE{Gezari1972ApJ...173L...1G,
    author = {{Gezari}, D.~Y. and {Labeyrie}, A. and {Stachnik}, R.~V.},
    title = "{Speckle Interferometry: Diffraction-Limited Measurements of Nine Stars with the 200-INCH Telescope}",
    journal = {\apjl},
    year = 1972,
    month = apr,
    volume = 173,
    pages = {L1},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1972ApJ...173L...1G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gezari1999yCat.2225....0G,
    author = {{Gezari}, D.~Y. and {Pitts}, P.~S. and {Schmitz}, M.},
    title = "{Catalog of Infrared Observations, Edition 5 (Gezari+ 1999)}",
    journal = {VizieR Online Data Catalog},
    year = 1999,
    month = jul,
    volume = 2225,
    pages = {0},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999yCat.2225....0G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gigas1986A&A...165..170G,
    author = {{Gigas}, D.},
    title = "The iron abundance of VEGA",
    journal = {\aap},
    year = 1986,
    month = sep,
    volume = 165,
    pages = {170--182},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...165..170G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Girardi2000A&AS..141..371G,
    author = {{Girardi}, L. and {Bressan}, A. and {Bertelli}, G. and {Chiosi}, C.
        },
    title = "Evolutionary tracks and isochrones for low- and intermediate-mass stars: From 0.15 to 7 M$_{\odot}$, and from Z=0.0004 to 0.03",
    journal = {\aaps},
    year = 2000,
    month = feb,
    volume = 141,
    pages = {371--383},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26AS..141..371G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Glass1974MNSSA..33...53G,
    author = {{Glass}, I.~S.},
    title = "{JHKL photometry of 145 southern stars.}",
    journal = {Monthly Notes of the Astronomical Society of South Africa},
    year = 1974,
    volume = 33,
    pages = {53--58},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1974MNSSA..33...53G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Glebocki1988A&A...189..199G,
    author = {{Glebocki}, R. and {Stawikowski}, A.},
    title = "Are tides responsible for enhanced MG II emission in late-type binaries?",
    journal = {\aap},
    year = 1988,
    month = jan,
    volume = 189,
    pages = {199--203},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988A%26A...189..199G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gliese1969VeARI..22....1G,
    author = {{Gliese}, W.},
    title = {Catalogue of Nearby Stars. Edition 1969},
    journal = {Ver\"{o}ffentlichungen des Astronomishen Rechen-Instituts Heidelberg},
    year = 1969,
    volume = 22,
    pages = {1},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1969VeARI..22....1G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Goldman1998,
        AUTHOR  = "{Goldman}, A. and {Schoenfeld}, W.\ G. and {Goorvitch},
                  D. and {Chackerian}, C.\ Jr. and {Dothe} H. and {M\'{e}len},
                  F. and {Abrams}, M.\ C. and {Selby}, J.\ E.\ A.",
        TITLE   = "Updated line parameters for OH X$^2\Pi$-X$^2\Pi$
                  $(v\prime\prime,v\prime)$ transitions",
        YEAR    = 1998,
        JOURNAL = jqsrt,
        VOLUME  = 59,
        PAGES   = "453--469"}



@ARTICLE{Gratton1982MNRAS.201..807G,
    author = {{Gratton}, L. and {Gaudenzi}, S. and {Rossi}, C. and {Gratton}, R.\ G.
        },
    title = "Studies on the spectra of K-giants. I - Physical parameters and Fe and Ti abundances for 26 K-giants",
    journal = {\mnras},
    year = 1982,
    month = dec,
    volume = 201,
    pages = {807--832},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.201..807G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gratton1983MNRAS.202..231G,
    author = {{Gratton}, R.\ G.},
    title = "Studies on the spectra of K-giants. II - Abundance determinations for K-giants from very strong iron lines",
    journal = {\mnras},
    year = 1983,
    month = jan,
    volume = 202,
    pages = {231--240},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983MNRAS.202..231G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gratton1985A&A...148..105G,
    author = {{Gratton}, R.\ G.},
    title = "Studies on the spectra of K-giants. III - Carbon, nitrogen, and oxygen abundances",
    journal = {\aap},
    year = 1985,
    month = jul,
    volume = 148,
    pages = {105--114},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985A%26A...148..105G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gray1975ApJ...202..148G,
    author = {{Gray}, D.\ F.},
    title = {Atmospheric turbulence measured in stars above the main sequence},
    journal = {\apj},
    year = 1975,
    month = nov,
    volume = 202,
    pages = {148--164},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975ApJ...202..148G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Gray1992,
    author = {{Gray}, D.\ F.},
    title = {The observation and analysis of stellar photospheres},
    publisher = {Cambridge Astrophysics Series, Cambridge: Cambridge University Press, 1992, 2nd ed., ISBN 0521403200.},
    year = 1992,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992oasp.book.....G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Grevesse1992RMxAA..23...71G,
    author = {{Grevesse}, N. and {Sauval}, A.\ J.},
    title = "Molecular Data from Solar Spectroscopy",
    journal = {Revista Mexicana de Astronomia y Astrofisica, vol.\ 23},
    year = 1992,
    month = mar,
    volume = 23,
    pages = {71},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992RMxAA..23...71G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Griffin1968,
    author = {{Griffin}, R.},
    title = "A photometric atlas of the spectrum of Arcturus, $\lambda \lambda 3600-8825$ {\AA}", 
    publisher = {Cambridge: Cambridge Philosophical Society, 1968},
    year = 1968,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1968pmas.book.....G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gunson1996GeoRL..23.2333G,
    author = {{Gunson}, M.\ R. and {Abbas}, M.\ M. and {Abrams}, M.\ C. and 
        {Allen}, M. and {Brown}, L.\ R. and {Brown}, T.\ L. and {Chang}, A.\ Y. and 
        {Goldman}, A. and {Irion}, F.\ W. and {Lowes}, L.\ L. and {Mahieu}, E. and 
        {Manney}, G.\ L. and {Michelsen}, H.\ A. and {Newchurch}, M.\ J. and 
        {Rinsland}, C.\ P. and {Salawitch}, R.\ J. and {Stiller}, G.\ P. and 
        {Toon}, G.\ C. and {Yung}, Y.\ L. and {Zander}, R.},
    title = "The atmospheric trace molecule spectroscopy (ATMOS) experiment: Deployment on the ATLAS Space Shuttle missions",
    journal = {\grl},
    year = 1996,
    volume = 23,
    pages = {2333},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996GeoRL..23.2333G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1974A&A....34...99G,
    author = {{Gustafsson}, B. and {Kj{\ae}rgaard}, P. and {Andersen}, S.},
    title = "The metal content and microturbulence in G8-K3 giants, as investigated by means of photoelectric photometry in very narrow bands.",
    journal = {\aap},
    year = 1974,
    month = aug,
    volume = 34,
    pages = {99--128},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974A%26A....34...99G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1975A&A....42..407G,
    author = {{Gustafsson}, B. and {Bell}, R.\ A. and {Eriksson}, K. and {Nordlund}, {\AA}.
        },
    title = {A grid of model atmospheres for metal-deficient giant stars. I},
    journal = {\aap},
    year = 1975,
    month = sep,
    volume = 42,
    pages = {407--432},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975A%26A....42..407G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1979A&A....74..313G,
    author = {{Gustafsson}, B. and {Bell}, R.~A.},
    title = "{The colours of G and K type giant stars. I}",
    journal = {\aap},
    year = 1979,
    month = may,
    volume = 74,
    pages = {313--352},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979A%26A....74..313G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1994A&ARv...6...19G,
    author = {{Gustafsson}, B. and {Jorgensen}, U.\ G.},
    title = "Models of late-type stellar photospheres",
    journal = {\aapr},
    year = 1994,
    month = nov,
    volume = 6,
    pages = {19--65},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26ARv...6...19G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hammersley1998A&AS..128..207H,
    author = {{Hammersley}, P.\ L. and {Jourdain de Muizon}, M. and {Kessler}, M.\ F. and 
        {Bouchet}, P. and {Joseph}, R.\ D. and {Habing}, H.\ J. and 
        {Salama}, A. and {Metcalfe}, L.},
    title = "Infrared standards for ISO. I. A new calibration of mid infrared photometry",
    journal = {\aaps},
    year = 1998,
    month = feb,
    volume = 128,
    pages = {207--219},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26AS..128..207H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Hammersley2001clim.confE..23H,
    author = {{Hammersley}, P.},
    title = "Development of Stellar Photometric Standards for ISO.",
    booktitle = {The calibration legacy of the {ISO} Mission},
    year = 2001,
    pages = {to be published},
    EDITOR    =  {{Metcalfe}, L. and {Kessler}, M.\ F.\ K.},   
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Harris1984ApJ...285..674H,
    author = {{Harris}, M.\ J. and {Lambert}, D.\ L.},
    title = "Oxygen isotopic abundances in the atmospheres of seven red giant stars",
    journal = {\apj},
    year = 1984,
    month = oct,
    volume = 285,
    pages = {674--682},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984ApJ...285..674H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Harris1988ApJ...325..768H,
    author = {{Harris}, M.\ J. and {Lambert}, D.\ L. and {Smith}, V.\ V.},
    title = "Oxygen isotopic abundances in evolved stars. IV - Five K giants",
    journal = {\apj},
    year = 1988,
    month = feb,
    volume = 325,
    pages = {768--775},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988ApJ...325..768H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Harwit2001ApJ...557..844H,
    author = {{Harwit}, M. and {Malfait}, K. and {Decin}, L. and {Waelkens}, C. and 
        {Feuchtgruber}, H. and {Melnick}, G.~J.},
    title = "{The Infrared Continuum Spectrum of VY Canis Majoris}",
    journal = {\apj},
    year = 2001,
    month = aug,
    volume = 557,
    pages = {844--853},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...557..844H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hill1993A&A...276..142H,
    author = {{Hill}, G.\ M. and {Landstreet}, J.\ D.},
    title = "Compositional Differences among the A-Type Stars - Part One - Six Narrowlined Stars",
    journal = {\aap},
    year = 1993,
    month = sep,
    volume = 276,
    pages = {142},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...276..142H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hill1995A&A...293..347H,
    author = {{Hill}, V. and {Andrievsky}, S. and {Spite}, M.},
    title = {Chemical evolution of the Magellanic Clouds. VI. Chemical composition of nine F supergiants from different regions of the large Magellanic Cloud.},
    journal = {\aap},
    year = 1995,
    month = jan,
    volume = 293,
    pages = {347--359},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...293..347H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hinkle1982ApJ...252..697H,
    author = {{Hinkle}, K.\ H. and {Hall}, D.\ N.\ B. and {Ridgway}, S.\ T.
        },
    title = "Time series infrared spectroscopy of the Mira variable Chi Cygni",
    journal = {\apj},
    year = 1982,
    month = jan,
    volume = 252,
    pages = {697--714},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...252..697H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hinkle1995PASP..107.1042H,
    author = {{Hinkle}, K. and {Wallace}, L. and {Livingston}, W.},
    title = {Infrared Atlas of the Arcturus Spectrum, 0.9-5.3 microns},
    journal = {\pasp},
    year = 1995,
    month = nov,
    volume = 107,
    pages = {1042},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995PASP..107.1042H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Hinkle1995,
        AUTHOR  = {{Hinkle}, K. and {Wallace}, L. and {Livingston}, W.},
        TITLE   = "Infrared Atlas of the Arcturus Spectrum, 0.9 -- 5.3 microns",
      PUBLISHER = "ASP, San Francisco",
        YEAR    = 1995
}




@BOOK{Hirhor95,
        AUTHOR  = {{Hirata}, R. and {Horaguchi}, T.},
        TITLE   = "Atomic spectral line list",
      PUBLISHER = "{internet: http://cdsweb.u-strasbg.fr/htbin/Cat?VI/69}",
        YEAR    = 1995,
        ADDRESS = ""}

@BOOK{Hoffleit1982,
    author = {{Hoffleit}, D. and {Jaschek}, C.},
    title = {The Bright Star Catalogue},
    publisher = {The Bright Star Catalogue, New Haven: Yale University Observatory (4th edition), 1982 },
    year = 1982,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982bsc..book.....H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{Hofner2001,                                       
        AUTHOR  = {{H\"{o}fner}, S. and {Loidl}, R. and {Aringer}, B. and {J{\o}rgensen}, U.}, 
        TITLE   = "Dynamical Atmospheres and Mass Loss of Pulsating AGB stars",
        BOOKTITLE = {ASP Conf. Ser.: Radial and Nonradial Pulsations as Probes of Stellar Physics},
        YEAR    = 2002,
        PAGES   = "{in press}",
      EDITOR    = "{Aerts}, C. and {Bedding}, T. and {Christensen-Dalsgaard}, J.",
      PUBLISHER = "{San Francisco: ASP}",
        ADDRESS = ""}


@ARTICLE{HolwegerMuller1974SoPh...39...19H,
    author = {{Holweger}, H. and {M\"{u}ller}, E.\ A.},
    title = {The photospheric barium spectrum - Solar abundance and collision broadening of BA II lines by hydrogen},
    journal = {\solphys},
    year = 1974,
    month = nov,
    volume = 39,
    pages = {19--30},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974SoPh...39...19H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Holweger1995A&A...303..819H,
    author = {{Holweger}, H. and {Rentzsch-Holm}, I.},
    title = {High-resolution spectroscopy of $\{$lambda$\}$ Bootis stars and `dusty' normal A stars: circumstellar gas, rotation, and accretion.},
    journal = {\aap},
    year = 1995,
    month = nov,
    volume = 303,
    pages = {819},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...303..819H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hui-Bon-Hoa1997A&A...323..901H,
    author = {{Hui-Bon-Hoa}, A. and {Burkhart}, C. and {Alecian}, G.},
    title = "Metal abundances of A-type stars in three galactic clusters.",
    journal = {\aap},
    year = 1997,
    month = jul,
    volume = 323,
    pages = {901--908},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...323..901H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hutter1989ApJ...340.1103H,
    author = {{Hutter}, D.\ J. and {Johnston}, K.\ J. and {Mozurkewich}, D. and 
        {Simon}, R.\ S. and {Colavita}, M.\ M. and {Pan}, X.\ P. and 
        {Shao}, M. and {Hines}, B.\ E. and {Staelin}, D.\ H. and {Hershey}, J.\ L. and 
        {Hughes}, J.\ A. and {Kaplan}, G.\ H.},
    title = "Angular diameter measurements of 24 giant and supergiant stars from the Mark III optical interferometer",
    journal = {\apj},
    year = 1989,
    month = may,
    volume = 340,
    pages = {1103--1111},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989ApJ...340.1103H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Iben1967ApJ...147..624I,
    author = {{Iben}, I.~J.},
    title = "{Stellar Evolution.VI. Evolution from the Main Sequence to the Red-Giant Branch for Stars of Mass 1 M\_$\{$sun$\}$, 1.25 M\_$\{$sun$\}$, and 1.5 M\_$\{$sun$\}$}",
    journal = {\apj},
    year = 1967,
    month = feb,
    volume = 147,
    pages = {624},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1967ApJ...147..624I&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Jenkins1952QB813.J45......,
    author = {{Jenkins}, L.\ F.},
    title = "General catalogue of trigonometric stellar parallaxes.",
    publisher = {New Haven, Yale University Observatory},
    year = 1952,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1952QB813.J45......&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Jenkins1963GCTP..C......0J,
    author = {{Jenkins}, L.~F.},
    title = "{Supplement to the General Catalogue of Trigonometric Stellar Parallaxes, Compiled at the Yale Univ. Obs.}",
    booktitle = {General Cat. Trigo. Parallaxes (1963)},
    year = 1963,
    pages = {0},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1963GCTP..C......0J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Johnson1966CoLPL...4...99J,
    author = {{Johnson}, H.~L. and {Iriarte}, B. and {Mitchell}, R.~I. and 
        {Wisniewskj}, W.~Z.},
    title = "{UBVRIJKL photometry of the bright stars.}",
    journal = {Communications of the Lunar and Planetary Laboratory},
    year = 1966,
    volume = 4,
    pages = {99},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1966CoLPL...4...99J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}




@ARTICLE{Jorgensen1992A&A...261..263J,
    author = {{J{\o}rgensen}, U.\ G. and {Johnson}, H.\ R. and
                  {Nordlund}, {\AA}.},
    title = "Effects of sphericity in carbon star atmospheres",
    journal = {\aap},
    year = 1992,
    month = jul,
    volume = 261,
    pages = {263--273},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...261..263J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Jorgensen1994mse..conf...29J,
    author = {{J{\o}rgensen}, U.\ G.},
    title = {Dominating Molecules in the Photosphere of Cool Stars},
    booktitle = {Molecules in the Stellar Environment, Proceedings of IAU Colloquium No. 146}, 
    year = 1994,
    pages = {29},
    EDITOR    = {{J{\o}rgensen}, U.\ G.},
        ADDRESS = "Springer-Verlag Berlin Heidelberg New York"}



@ARTICLE{Justtanont1998A&A...330L..17J,
    author = {{Justtanont}, K. and {Feuchtgruber}, H. and {de Jong}, T. and 
        {Cami}, J. and {Waters}, L.\ B.\ F.\ M. and {Yamamura}, I. and 
        {Onaka}, T.},
    title = "Discovery of CO\_2 emission in AGB stars  with the 13mu M dust feature",
    journal = {\aap},
    year = 1998,
    month = feb,
    volume = 330,
    pages = {L17--L20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...330L..17J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kamper1978AJ.....83.1653K,
    author = {{Kamper}, K.\ W. and {Wesselink}, A.\ J.},
    title = {Alpha and Proxima Centauri},
    journal = {\aj},
    year = 1978,
    month = dec,
    volume = 83,
    pages = {1653--1659},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978AJ.....83.1653K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Kelly1983,
        AUTHOR  = "{Kelly}, R.\ L.",
        TITLE   = "Unpublished work",
        PUBLISHER = {magnetic tape},
        YEAR    = 1983,
        ADDRESS = ""}

@INPROCEEDINGS{Kester2001clim.confE..46K,
    author = {{Kester}, D. and {Fouks}, B. and {Lahuis}, F.},
    title = "{SWS Transient Effects: Models and Corrections}",
    booktitle = {The Calibration Legacy of the ISO Mission},
    year = 2001,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001clim.confE..46K&db_key=AST},
    PAGES   = {46},
    EDITOR    = {{Metcalfe}, L. and {Kessler}, F.\ K.},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kjaergaard1982A&A...115..145K,
    author = {{Kj{\ae}rgaard}, P. and {Gustafsson}, B. and {Walker}, G.\ A.\ H. and 
        {Hultqvist}, L.},
    title = "Carbon, nitrogen, and oxygen abundances in G8-K3 giant stars",
    journal = {\aap},
    year = 1982,
    month = nov,
    volume = 115,
    pages = {145--163},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982A%26A...115..145K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Koechlin1985A&A...153...91K,
    author = {{Koechlin}, L. and {Rabbia}, Y.},
    title = "Stellar diameter measurements with the CERGA optical interferometer - Recent developments and results",
    journal = {\aap},
    year = 1985,
    month = dec,
    volume = 153,
    pages = {91--98},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985A%26A...153...91K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kovacs1983A&A...120...21K,
    author = {{Kov\'{a}cs}, N.},
    title = "{Model-atmosphere analysis of high-dispersion spectra of four red giants and supergiants}",
    journal = {\aap},
    year = 1983,
    month = apr,
    volume = 120,
    pages = {21--35},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983A%26A...120...21K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Kupka1999A&AS..138..119K,
    author = {{Kupka}, F. and {Piskunov}, N. and {Ryabchikova}, T.\ A. and 
        {Stempels}, H.\ C. and {Weiss}, W.\ W.},
    title = {VALD-2: Progress of the Vienna Atomic Line Data Base},
    journal = {\aaps},
    year = 1999,
    month = jul,
    volume = 138,
    pages = {119--133},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26AS..138..119K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1970SAOSR.308.....K,
    author = {{Kurucz}, R.\ L.},
    title = "Atlas: a Computer Program for Calculating Model Stellar Atmospheres",
    journal = {SAO Special Report},
    year = 1970,
    month = feb,
    volume = 308,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1970SAOSR.308.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1975SAOSR.362.....K,
    author = {{Kurucz}, R.\ L. and {Peytremann}, E.},
    title = {A table of semiempirical gf values.  Part 1: Wavelengths:  5.2682 NM to 272.3380 NM},
    journal = {SAO Special Report},
    year = 1975,
    month = feb,
    volume = 362,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975SAOSR.362.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Kurucz1979ApJS...40....1K,
    author = {{Kurucz}, R.\ L.},
    title = "Model atmospheres for G, F, A, B, and O stars",
    journal = {\apjs},
    year = 1979,
    month = may,
    volume = 40,
    pages = {1 -- 340},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJS...40....1K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Kurucz1979Smith,
        AUTHOR  = {{Kurucz}, R.\ L. and {Furenlid}, I.},
        TITLE   = "",
        YEAR    = 1979,
        JOURNAL = {Smithsonian Astrophys.\ Obs.\ Spec.\ Rept.},
        VOLUME  = {387},
        PAGES   = ""}


@BOOK{Kurucz1989,
        AUTHOR  = "{Kurucz}, R.\ L.",
        TITLE   = "New gf-calculations",
        PUBLISHER = {magnetic tape},
        YEAR    = 1989,
        ADDRESS = ""}

@INPROCEEDINGS{Kurucz1991sabc.conf..441K,
    author = {{Kurucz}, R.\ L.},
    title = "New Opacity Calculations",
    booktitle = {Stellar Atmospheres: Beyond Classical Models, Proceedings of the Advanced Research Workshop.},  
    year = 1991,
    pages = {441},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991sabc.conf..441K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1992RMxAA..23...45K,
    author = {{Kurucz}, R.\ L.},
    title = "Atomic and Molecular Data for Opacity Calculations",
    journal = {Revista Mexicana de Astronomia y Astrofisica},
    year = 1992,
    month = mar,
    volume = 23,
    pages = {45},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992RMxAA..23...45K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1993KurCD..13.....K,
    author = {{Kurucz}, R.},
    title = "ATLAS9 Stellar Atmosphere Programs and 2 km/s grid.",
    journal = {ATLAS9 Stellar Atmosphere Programs and 2 km/s grid.\ Kurucz CD-ROM No.\ 13.\  Cambridge, MA: Smithsonian Astrophysical Observatory},
    year = 1993,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993KurCD..13.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Kurucz1993sssp.book.....K,
    author = {{Kurucz}, R.\ L.},
    title = "SYNTHE spectrum synthesis programs and line data",
    publisher = {Kurucz CD-ROM, Cambridge, MA: Smithsonian Astrophysical Observatory},
    year = 1993,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993sssp.book.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kyrolainen1986A&AS...65...11K,
    author = {{Kyr\"{o}l\"{a}inen}, J. and {Tuominen}, I. and {Vilhu}, O. and {Virtanen}, H.
        },
    title = "Optical spectroscopy of eleven G- and K-giants",
    journal = {\aaps},
    year = 1986,
    month = jul,
    volume = 65,
    pages = {11--20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26AS...65...11K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Lambert1976MSRSL...9..405L,
    author = {{Lambert}, D.~L.},
    title = "{The C-12/C-13 ratio in late-type stellar atmospheres}",
    journal = {Memoires of the Societe Royale des Sciences de Liege},
    year = 1976,
    volume = 9,
    pages = {405--415},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976MSRSL...9..405L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1980ApJ...235..114L,
    author = {{Lambert}, D.\ L. and {Dominy}, J.\ F. and {Sivertsen}, S.},
    title = "Lithium in late-type giants. I - G and K giants",
    journal = {\apj},
    year = 1980,
    month = jan,
    volume = 235,
    pages = {114--125},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJ...235..114L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1981ApJ...248..228L,
    author = {{Lambert}, D.\ L. and {Ries}, L.\ M.},
    title = "Carbon, nitrogen, and oxygen abundances in G and K giants",
    journal = {\apj},
    year = 1981,
    month = aug,
    volume = 248,
    pages = {228--248},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...248..228L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1982ApJ...254..663L,
    author = {{Lambert}, D.\ L. and {Roby}, S.\ W. and {Bell}, R.\ A.},
    title = "Carbon, nitrogen, and oxygen abundances in Sirius and VEGA",
    journal = {\apj},
    year = 1982,
    month = mar,
    volume = 254,
    pages = {663--669},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...254..663L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1987Ap&SS.133..369L,
    author = {{Lambert}, D.\ L. and {McWilliam}, A. and {Smith}, V.\ V.},
    title = "Isotopic abundances of silicon in four red giants",
    journal = {\apss},
    year = 1987,
    month = may,
    volume = 133,
    pages = {369--381},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987Ap%26SS.133..369L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lamers1994A&A...291..856L,
    author = {{Lamers}, H.\ J.\ G.\ L.\ M. and {Achmad}, L.},
    title = {The relation between microturbulence and mass loss from supergiants},
    journal = {\aap},
    year = 1994,
    month = nov,
    volume = 291,
    pages = {856--868},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...291..856L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lane1984ApJ...281..723L,
    author = {{Lane}, M.\ C. and {Lester}, J.\ B.},
    title = "Effective temperatures and surface gravities of metallic-line A stars",
    journal = {\apj},
    year = 1984,
    month = jun,
    volume = 281,
    pages = {723--738},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984ApJ...281..723L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Langhoff1989,
        AUTHOR  = {{Langhoff}, S.\ R. and {Bauschlicher}, C.\ W.\ Jr.},
        TITLE   = { },
        YEAR    = 1989,
        JOURNAL = {J. Chem. Phys.},
        VOLUME  = 91,
        PAGES   = "5953"}

@ARTICLE{Langhoff1993,
        AUTHOR  = {{Langhoff}, S.\ R. and {Bauschlicher}, C.\ W.\ Jr.},
        TITLE   = { },
        YEAR    = 1993,
        JOURNAL = {Chem. Phys. Letters},
        VOLUME  = 211,
        PAGES   = "305"}

@ARTICLE{Lazaro1991MNRAS.249...62L,
    author = {{Lazaro}, C. and {Lynas-Gray}, A.\ E. and {Clegg}, R.\ E.\ S. and 
        {Mountain}, C.\ M. and {Zadrozny}, A.},
    title = "Carbon abundances and isotope ratios in 70 bright M giants",
    journal = {\mnras},
    year = 1991,
    month = mar,
    volume = 249,
    pages = {62--68},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991MNRAS.249...62L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lee1970ApJ...162..217L,
    author = {{Lee}, T.~A.},
    title = "{Photometry of high-luminosity M-type stars}",
    journal = {\apj},
    year = 1970,
    month = oct,
    volume = 162,
    pages = {217},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1970ApJ...162..217L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Leech2002,                                       
        AUTHOR  = "{Leech}, K. and {Kester}, D. and {Shipman}, R. and {Beintema}, D. and {Feuchtgruber}, H. and {Heras}, A. and {Huygen}, R. and {Lahuis}, F. and {Lutz}, D. and {Morris}, P. and {Roelfsema}, P. and {Salama}, A. and {Schaeidt}, S. and {Valentijn}, E. and {Vandenbussche}, B. and {Wieprecht}, E. and {de Graauw} T.", 
        TITLE   = "SWS --- The Short Wavelength Spectrometer",
        BOOKTITLE = "The ISO Handbook. Volume V. SWS - The Short Wavelength 
                     Spectrometer",     
        YEAR    = 2002,
      EDITOR    = "{Leech}, K."}


@ARTICLE{Leggett1986A&A...159..217L,
    author = {{Leggett}, S.\ K. and {Mountain}, C.\ M. and {Selby}, M.\ J. and 
        {Blackwell}, D.\ E. and {Booth}, A.\ J. and {Haddock}, D.\ J. and 
        {Petford}, A.\ D.},
    title = "The effective temperatures, diameters and luminosities of 22 bright stars by application of the infrared flux method",
    journal = {\aap},
    year = 1986,
    month = apr,
    volume = 159,
    pages = {217--222},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...159..217L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lejeune2001A&A...366..538L,
    author = {{Lejeune}, T. and {Schaerer}, D.},
    title = "{Database of Geneva stellar evolution tracks and isochrones  for (UBV)<SUB>J</SUB>(RI)<SUB>C</SUB> JHKLL'M, HST-WFPC2, Geneva   and Washington photometric systems}",
    journal = {\aap},
    year = 2001,
    month = feb,
    volume = 366,
    pages = {538--546},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001A%26A...366..538L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}
@ARTICLE{Lemke1990A&A...240..331L,
    author = {{Lemke}, M.},
    title = "Abundance anomalies in main sequence A stars. II - C, Si, CA and the heavy elements SR and BA",
    journal = {\aap},
    year = 1990,
    month = dec,
    volume = 240,
    pages = {331--345},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26A...240..331L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lester1986ApJS...61..509L,
    author = {{Lester}, J.\ B. and {Gray}, R.\ O. and {Kurucz}, R.\ L.},
    title = {Theoretical uvby-beta indices},
    journal = {\apjs},
    year = 1986,
    month = jul,
    volume = 61,
    pages = {509--529},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986ApJS...61..509L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Linsky1978ApJ...220..619L,
    author = {{Linsky}, J.\ L. and {Ayres}, T.\ R.},
    title = {Stellar model chromospheres. VI - Empirical estimates of the chromospheric radiative losses of late-type stars},
    journal = {\apj},
    year = 1978,
    month = mar,
    volume = 220,
    pages = {619--628},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...220..619L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Linsky1979ApJS...41...47L,
    author = {{Linsky}, J.~L. and {McClintock}, W. and {Robertson}, R.~M. and 
        {Worden}, S.~P.},
    title = "{Stellar model chromospheres. X - High-resolution, absolute flux profiles of the CA II H and K lines in stars of spectral types F0-M2}",
    journal = {\apjs},
    year = 1979,
    month = sep,
    volume = 41,
    pages = {47--74},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJS...41...47L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Lorente1998,
        AUTHOR  = "{Lorente}, R.",
        TITLE   = {Spectral Resolution of SWS AOT 1},
      PUBLISHER = {ISO-SWS online documentation, http://sws.ster.kuleuven.ac.be},
        YEAR    = 1998}


@ARTICLE{Luck1979ApJ...232..797L,
    author = {{Luck}, R.\ E.},
    title = {The chemical compositions of nine southern supergiant stars},
    journal = {\apj},
    year = 1979,
    month = sep,
    volume = 232,
    pages = {797--806},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...232..797L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Luck1985ApJ...298..782L,
    author = {{Luck}, R.\ E. and {Lambert}, D.\ L.},
    title = {Carbon, nitrogen, and oxygen in intermediate-mass supergiants - Is oxygen underabundant?},
    journal = {\apj},
    year = 1985,
    month = nov,
    volume = 298,
    pages = {782--802},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985ApJ...298..782L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Luck1995AJ....110.2968L,
    author = {{Luck}, R.\ E. and {Challener}, S.\ L.},
    title = "Chemical Abundances for Very Strong-Lined Giants",
    journal = {\aj},
    year = 1995,
    month = dec,
    volume = 110,
    pages = {2968},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995AJ....110.2968L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Lutz1999,
        AUTHOR  = "{Lutz}, D. and {Feuchtgruber}, H. and {Morfill}, J.",
        TITLE   = {ISO-SWS grating resolution and instrumental profile as
                  measured by the full resolution modes SWS02 and SWS06},
      PUBLISHER = "ISO-SWS online documentation, http://sws.ster.kuleuven.ac.be",
        YEAR    = 1999},

@ARTICLE{Lyubimkov1984Ap.....19..385L,
    author = {{Lyubimkov}, L.\ S. and {Boyarchuk}, A.\ A.},
    title = {Influence of Deviations from Local Thermodynamics Equilibrium on the Determination of Microturbulence in the Atmospheres of F-Type Supergiants},
    journal = {Astrophysics},
    year = 1984,
    volume = 19,
    pages = {385},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984Ap.....19..385L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mackle1975A&AS...19..303M,
    author = {{M{\"a}ckle}, R. and {Griffin}, R. and {Griffin}, R. and {Holweger}, H.
        },
    title = "A model-atmosphere analysis of the spectrum of Arcturus (basic spectroscopic data)",
    journal = {\aaps},
    year = 1975,
    month = mar,
    volume = 19,
    pages = {303},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975A%26AS...19..303M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Malagnini1986A&A...162..140M,
    author = {{Malagnini}, M.\ L. and {Morossi}, C. and {Rossi}, L. and {Kurucz}, R.\ L.
        },
    title = "The empirical BC versus T(eff) scale for non-supergiant O9-G5 stars",
    journal = {\aap},
    year = 1986,
    month = jul,
    volume = 162,
    pages = {140--150},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...162..140M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Malagnini1990A&AS...85.1015M,
    author = {{Malagnini}, M.\ L. and {Morossi}, C.},
    title = {Accurate absolute luminosities, effective temperatures, radii, masses and surface gravities for a selected sample of field stars},
    journal = {\aaps},
    year = 1990,
    month = nov,
    volume = 85,
    pages = {1015--1019},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26AS...85.1015M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Malagnini1997A&A...326..736M,
    author = {{Malagnini}, M.\ L. and {Morossi}, C.},
    title = {Accuracy of effective temperatures of solar chemical composition stars derived from the flux fitting method.},
    journal = {\aap},
    year = 1997,
    month = oct,
    volume = 326,
    pages = {736--740},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...326..736M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Manduca1979A&AS...36..411M,
    author = {{Manduca}, A.},
    title = "{Infrared Limb-Darkening Coefficients for Late-Type Giant Model Atmospheres}",
    journal = {\aaps},
    year = 1979,
    month = jun,
    volume = 36,
    pages = {411},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979A%26AS...36..411M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Manduca1981ApJ...243..883M,
    author = {{Manduca}, A. and {Bell}, R.\ A. and {Gustafsson}, B.},
    title = "The analysis of infrared fluxes of some late-type stars",
    journal = {\apj},
    year = 1981,
    month = feb,
    volume = 243,
    pages = {883--893},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...243..883M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mathis1990ARA&A..28...37M,
    author = {{Mathis}, J.~S.},
    title = "{Interstellar dust and extinction}",
    journal = {\araa},
    year = 1990,
    volume = 28,
    pages = {37--70},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ARA%26A..28...37M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mauron1992A&A...265..711M,
    author = {{Mauron}, N. and {Caux}, E.},
    title = "K I/Na I scattering observations in circumstellar envelopes - Alpha(1) Herculis, Omicron Ceti, TX PISCIUM and Beta Pegasi",
    journal = {\aap},
    year = 1992,
    month = nov,
    volume = 265,
    pages = {711--725},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...265..711M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mauron1995A&A...298..869M,
    author = {{Mauron}, N. and {Guilain}, C.},
    title = "NaI and KI scattering in circumstellar envelopes: new detections around giants and the NaI $\{$lambda$\}$5896/KI $\{$lambda$\}$7699 line ratio.",
    journal = {\aap},
    year = 1995,
    month = jun,
    volume = 298,
    pages = {869},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...298..869M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{McWilliam1990ApJS...74.1075M,
    author = {{McWilliam}, A.},
    title = {High-resolution spectroscopic survey of 671 GK giants. I - Stellar atmosphere parameters and abundances},
    journal = {\apjs},
    year = 1990,
    month = dec,
    volume = 74,
    pages = {1075--1128},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJS...74.1075M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mendoza1967BOTT....4..106M,
    author = {{Mendoza}, E.~E.},
    title = "{UBVRI photometry of southern bright stars}",
    journal = {Boletin de los Observatorios Tonantzintla y Tacubaya},
    year = 1967,
    volume = 4,
    pages = {106},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1967BOTT....4..106M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mendoza1969BOTT....5...57M,
    author = {{Mendoza}, E.~E.},
    title = "{BVRI photometry of 46 southern bright stars}",
    journal = {Boletin de los Observatorios Tonantzintla y Tacubaya},
    year = 1969,
    volume = 5,
    pages = {57},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1969BOTT....5...57M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Melen1995,
        AUTHOR  = "{M\'{e}len}, F. and {Sauval}, A.\ J. and {Grevesse}, N. and
                  {Farmer}, C.\ B. and {Servais}, C. and {Delbouille}, L. and
                  {Roland}, G.",
        TITLE   = "A new analysis of the OH radical spectrum from solar infrared
                  observations", 
        YEAR    = 1995,
        JOURNAL = jmolspec,
        VOLUME  = 174,
        PAGES   = "490--509"}

@BOOK{Mermilliod1986EgUBV.........M,
    author = {{Mermilliod}, J.-C.},
    title = "{Compilation of Eggen's UBV data, transformed to UBV}",
    journal = {Catalogue of Eggen's UBV data.~(1986)},
    year = 1986,
    publisher = {SIMBAD},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1986EgUBV.........M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Mihalas,
        AUTHOR  = "{Mihalas}, D.",
        TITLE   = "Stellar Atmospheres",
      PUBLISHER = "W.H. Freeman and Company",
        YEAR    = 1978,
        ADDRESS = ""}



@ARTICLE{Monnier1998ApJ...502..833M,
    author = {{Monnier}, J.\ D. and {Geballe}, T.\ R. and {Danchi}, W.\ C.
        },
    title = {Temporal Variations of Midinfrared Spectra in Late-Type Stars},
    journal = {\apj},
    year = 1998,
    month = aug,
    volume = 502,
    pages = {833},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998ApJ...502..833M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Moon1985Ap&SS.117..261M,
    author = {{Moon}, T.},
    title = {Stellar luminosities and radii from uvby-beta photometry},
    journal = {\apss},
    year = 1985,
    month = dec,
    volume = 117,
    pages = {261--270},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985Ap%26SS.117..261M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Moon1985MNRAS.217..305M,
    author = {{Moon}, T.\ T. and {Dworetsky}, M.\ M.},
    title = {Grids for the determination of effective temperature and surface gravity of B, A and F stars using uvby-beta photometry},
    journal = {\mnras},
    year = 1985,
    month = nov,
    volume = 217,
    pages = {305--315},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985MNRAS.217..305M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Morossi1993A&A...277..173M,
    author = {{Morossi}, C. and {Franchini}, M. and {Malagnini}, M.\ L. and 
        {Kurucz}, R.\ L. and {Buser}, R.},
    title = "Cool Stars - Spectral Energy Distributions and Model Atmosphere Fluxes",
    journal = {\aap},
    year = 1993,
    month = sep,
    volume = 277,
    pages = {173},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...277..173M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Morton1991ApJS...77..119M,
    author = {{Morton}, D.\ C.},
    title = {Atomic data for resonance absorption lines. I - Wavelengths longward of the Lyman limit},
    journal = {\apjs},
    year = 1991,
    month = sep,
    volume = 77,
    pages = {119--202},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991ApJS...77..119M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Morton1992ApJS...81..883M,
    author = {{Morton}, D.\ C.},
    title = {Atomic Data for Resonance Absorption Lines. I. Wavelengths Longward of the Lyman Limit: Erratum},
    journal = {\apjs},
    year = 1992,
    month = aug,
    volume = 81,
    pages = {883},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992ApJS...81..883M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mozurkewich1991AJ....101.2207M,
    author = {{Mozurkewich}, D. and {Johnston}, K.\ J. and {Simon}, R.\ S. and 
        {Bowers}, P.\ F. and {Gaume}, R. and {Hutter}, D.\ J. and {Colavita}, M.\ M. and 
        {Shao}, M. and {Pan}, X.\ P.},
    title = "Angular diameter measurements of stars",
    journal = {\aj},
    year = 1991,
    month = jun,
    volume = 101,
    pages = {2207--2219},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991AJ....101.2207M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Napiwotzki1993A&A...268..653N,
    author = {{Napiwotzki}, R. and {Sch\"{o}nberner}, D. and {Wenske}, V.},
    title = {On the determination of effective temperature and surface gravity of B, A, and F stars using Stromgren UVBY beta photometry},
    journal = {\aap},
    year = 1993,
    month = feb,
    volume = 268,
    pages = {653--666},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...268..653N&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Neuforge1997A&A...328..261N,
    author = {{Neuforge-Verheecke}, C. and {Magain}, P.},
    title = {Spectroscopic analysis of the Alpha Centauri system},
    journal = {\aap},
    year = 1997,
    month = dec,
    volume = 328,
    pages = {261--268},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...328..261N&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Nicolet1978A&AS...34....1N,
    author = {{Nicolet}, B.},
    title = "{Photoelectric photometric catalogue of homogeneous measurements in the UBV system.}",
    journal = {\aaps},
    year = 1978,
    month = oct,
    volume = 34,
    pages = {1--49},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1978A%26AS...34....1N&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Oinas1977A&A....61...17O,
    author = {{Oinas}, V.},
    title = "Neutral-ion anomaly in cool stars",
    journal = {\aap},
    year = 1977,
    month = oct,
    volume = 61,
    pages = {17--20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1977A%26A....61...17O&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Partridge+Schwenke1995,
        AUTHOR  = "{Partridge}, H. and {Schwenke}, D.\ W.",
        TITLE   = "The determination of an accurate isotope dependent potential
                  energy surface for water from extensive ab initio calculations
                  and experimental data",
        YEAR    = 1997,
        JOURNAL = jchemp,
        VOLUME  = 106,
        PAGES   = "4618--4639"}

@ARTICLE{Pasquini1990A&A...234..277P,
    author = {{Pasquini}, L. and {Brocato}, E. and {Pallavicini}, R.},
    title = "{Chromospheric activity of evolved late-type stars - Chromospheric activity in evolved stars}",
    journal = {\aap},
    year = 1990,
    month = aug,
    volume = 234,
    pages = {277--283},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26A...234..277P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Pasquini1992A&A...266..340P,
    author = {{Pasquini}, L. and {Brocato}, E.},
    title = "Chromospheric activity and stellar evolution - Clues from IUE data",
    journal = {\aap},
    year = 1992,
    month = dec,
    volume = 266,
    pages = {340--346},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...266..340P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Perrin1998A&A...331..619P,
    author = {{Perrin}, G. and {Coude Du Foresto}, V. and {Ridgway}, S.\ T. and 
        {Mariotti}, J.\ -. and {Traub}, W.\ A. and {Carleton}, N.\ P. and 
        {Lacasse}, M.\ G.},
    title = "Extension of the effective temperature scale  of giants to types later than M6",
    journal = {\aap},
    year = 1998,
    month = mar,
    volume = 331,
    pages = {619--626},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...331..619P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Peterson1993ApJ...404..333P,
    author = {{Peterson}, R.\ C. and {Dalle Ore}, C.\ M. and {Kurucz}, R.\ L.
        },
    title = "The nonsolar abundance ratios of Arcturus deduced from spectrum synthesis",
    journal = {\apj},
    year = 1993,
    month = feb,
    volume = 404,
    pages = {333--347},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...404..333P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Pilachowski1997AJ....114..819P,
    author = {{Pilachowski}, C. and {Sneden}, C. and {Hinkle}, K. and {Joyce}, R.
        },
    title = "Carbon Isotope Ratios from the First Overtone CO Bands in Metal-Poor Giants.",
    journal = {\aj},
    year = 1997,
    month = aug,
    volume = 114,
    pages = {819--824},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997AJ....114..819P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Piskunov1995lahr.conf..610P,
    author = {{Piskunov}, N.\ E. and {Kupka}, F. and {Ryabchikova}, T.\ A. and 
        {Weiss}, W.\ W. and {Jeffery}, C.\ S.},
    title = {The Vienna Atomic Line Data-Base},
    booktitle = {ASP Conf. Ser. 81: Laboratory and Astronomical High Resolution Spectra},
    year = 1995,
    pages = {610},
     EDITOR    = {{Sauval}, A.\ J. and {Blomme}, R. and {Grevesse}, N.},
        ADDRESS = "ASP"}



@ARTICLE{Plez1992A&A...256..551P ,
    author = {{Plez}, B. and {Brett}, J.\ M. and {Nordlund}, {\AA}.},
    title = {Spherical opacity sampling model atmospheres for M-giants. I - Techniques, data and discussion},
    journal = {\aap},
    year = 1992,
    month = mar,
    volume = 256,
    pages = {551--571},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...256..551P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Plez1993ApJ...418..812P,
    author = {{Plez}, B. and {Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = {Lithium Abundances and Other Clues to Envelope Burning in Small Magellanic Cloud Asymptotic Giant Branch Stars},
    journal = {\apj},
    year = 1993,
    month = dec,
    volume = 418,
    pages = {812},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...418..812P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Popper1980ARA&A..18..115P,
    author = {{Popper}, D.~M.},
    title = "{Stellar masses}",
    journal = {\araa},
    year = 1980,
    volume = 18,
    pages = {115--164},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ARA%26A..18..115P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Popper1993ApJ...404L..67P,
    author = {{Popper}, D.\ M.},
    title = {Main-sequence G and K stellar masses},
    journal = {\apjl},
    year = 1993,
    month = feb,
    volume = 404,
    pages = {L67--L70},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...404L..67P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Pottasch1992A&A...264..138P,
    author = {{Pottasch}, E.\ M. and {Butcher}, H.\ R. and {van Hoesel}, F.\ H.\ J.
        },
    title = {Solar-like oscillations on Alpha Centauri A},
    journal = {\aap},
    year = 1992,
    month = oct,
    volume = 264,
    pages = {138--146},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...264..138P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Pourbaix1999A&A...344..172P,
    author = {{Pourbaix}, D. and {Neuforge-Verheecke}, C. and {Noels}, A.},
    title = {Revised masses of alpha  Centauri},
    journal = {\aap},
    year = 1999,
    month = apr,
    volume = 344,
    pages = {172--176},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...344..172P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Price1968AJ.....73..431P,
    author = {{Price}, S.~D.},
    title = "{Results of an infrared stellar survey.}",
    journal = {\aj},
    year = 1968,
    month = aug,
    volume = 73,
    pages = {431},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1968AJ.....73..431P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Qiu2001Apj...548...953Q,
    author = {{Qiu}, H.\M. and {Zhao}, G. and {Chen}, Y.\ Q. and {Li}, Z.\ W.},
    title = "The abundance patterns of Sirius and Vega",
    journal = {\aap},
    year = 2001,
    month = feb,
    volume = 548,
    pages = {953--965},
    url = {},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Quirrenbach1993ApJ...406..215Q,
    author = {{Quirrenbach}, A. and {Mozurkewich}, D. and {Armstrong}, J.\ T. and 
        {Buscher}, D.\ F. and {Hummel}, C.\ A.},
    title = "Angular diameter measurements of cool giant stars in strong TiO bands and in the continuum",
    journal = {\apj},
    year = 1993,
    month = mar,
    volume = 406,
    pages = {215--219},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...406..215Q&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Quirrenbach1996A&A...312..160Q,
    author = {{Quirrenbach}, A. and {Mozurkewich}, D. and {Buscher}, D.\ F. and 
        {Hummel}, C.\ A. and {Armstrong}, J.\ T.},
    title = "Angular diameter and limb darkening of Arcturus.",
    journal = {\aap},
    year = 1996,
    month = aug,
    volume = 312,
    pages = {160--166},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...312..160Q&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Rentzsch-Holm1997A&A...317..178R,
    author = {{Rentzsch-Holm}, I.},
    title = "Abundance anomalies in main sequence A stars. III. Nitrogen and sulphur.", 
    journal = {\aap},
    year = 1997,
    month = jan,
    volume = 317,
    pages = {178--184},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...317..178R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ridgway1980ApJ...235..126R,
    author = {{Ridgway}, S.~T. and {Joyce}, R.~R. and {White}, N.~M. and {Wing}, R.~F.
        },
    title = "{Effective temperatures of late-type stars - The field giants from K0 to M6}",
    journal = {\apj},
    year = 1980,
    month = jan,
    volume = 235,
    pages = {126--137},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJ...235..126R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@PHDTHESIS{Ries1981,
    author = {{Ries}, L.\ M.},
    title = {Carbon, nitrogen, and oxygen abundances in G and K giants},
    school = {Texas Univ., Arlington.},
    year = 1981,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981PhDT.........4R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Robinson1998ApJ...503..396R,
    author = {{Robinson}, R.\ D. and {Carpenter}, K.\ G. and {Brown}, A.},
    title = "Goddard High-Resolution Spectrograph Observations of Cool Low-Gravity Stars. IV. A Comparison of the K5 III Stars alpha Tauri and gamma Draconis",
    journal = {\apj},
    year = 1998,
    month = aug,
    volume = 503,
    pages = {396},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998ApJ...503..396R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Roby1990ApJS...73...67R,
    author = {{Roby}, S.\ W. and {Lambert}, D.\ L.},
    title = "Carbon, nitrogen, and oxygen abundances in the chemically peculiar stars of the upper main sequence",
    journal = {\apjs},
    year = 1990,
    month = may,
    volume = 73,
    pages = {67--0049},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJS...73...67R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Rodgers1991ApJ...382..606R,
    author = {{Rodgers}, B. and {Glassgold}, A.\ E.},
    title = "The temperature of the circumstellar envelope of Alpha Orionis",
    journal = {\apj},
    year = 1991,
    month = dec,
    volume = 382,
    pages = {606--616},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991ApJ...382..606R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Russell1989ApJS...70..865R,
    author = {{Russell}, S.\ C. and {Bessell}, M.\ S.},
    title = {Abundances of the heavy elements in the Magellanic Clouds. I - Metal abundances of F-type supergiants},
    journal = {\apjs},
    year = 1989,
    month = aug,
    volume = 70,
    pages = {865--898},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989ApJS...70..865R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Reader1980wtpa.book.....R,
    author = {{Reader}, J. and {Corliss}, C.\ H. and {Wiese}, W.\ L. and {Martin}, G.\ A.
        },
    title = {Wavelengths and transition probabilities for atoms and atomic ions - Part 1: Wavelengths - Part 2: Transition probabilities},
    publisher = {NSRDS-NBS 68, Washington},
    year = 1980,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980wtpa.book.....R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Relyea1978ApJS...37...45R,
    author = {{Relyea}, L.\ J. and {Kurucz}, R.\ L.},
    title = "A theoretical analysis of UVBY photometry",
    journal = {\apjs},
    year = 1978,
    month = may,
    volume = 37,
    pages = {45--69},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJS...37...45R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@PHDTHESIS{Ries1981PhDT.........4R,
    author = {{Ries}, L.\ M.},
    title = "Carbon, nitrogen, and oxygen abundances in G and K giants",
    school = {Texas Univ., Arlington.},
    year = 1981,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981PhDT.........4R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ryabchikova1997BaltA...6..244R,
    author = {{Ryabchikova}, T.\ A. and {Piskunov}, N.\ E. and {Kupka}, F. and 
        {Weiss}, W.\ W.},
    title = {The Vienna Atomic Line Database : Present State and Future Development},
    journal = {Baltic Astronomy},
    year = 1997,
    month = mar,
    volume = 6,
    pages = {244--247},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997BaltA...6..244R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ryde1999A&A...341..579R,
    author = {{Ryde}, N. and {Eriksson}, K. and {Gustafsson}, B.},
    title = "The nature of the circumstellar CO\_2 emission from M giants",
    journal = {\aap},
    year = 1999,
    month = jan,
    volume = 341,
    pages = {579--586},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...341..579R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sadakane1981PASJ...33..189S,
    author = {{Sadakane}, K. and {Nishimura}, M.},
    title = "Metal Abundances and the Microturbulence in VEGA",
    journal = {\pasj},
    year = 1981,
    volume = 33,
    pages = {189},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981PASJ...33..189S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sadakane1989PASJ...41..279S,
    author = {{Sadakane}, K. and {Ueta}, M.},
    title = "Abundance analysis of Sirius in the blue-violet region",
    journal = {\pasj},
    year = 1989,
    volume = 41,
    pages = {279--288},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989PASJ...41..279S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sanner1976ApJS...32..115S,
    author = {{Sanner}, F.},
    title = "Mass loss in red giants and supergiants",
    journal = {\apjs},
    year = 1976,
    month = sep,
    volume = 32,
    pages = {115--145},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJS...32..115S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@BOOK{Sauval2000,
        AUTHOR  = {{Sauval}, A.\ J.},
        TITLE   = "Data file of IR solar atomic lines",
      PUBLISHER = {unpublished results},
        YEAR    = 2002,
        ADDRESS = ""}


@ARTICLE{Scalo1976ApJ...206..474S,
    author = {{Scalo}, J.~M.},
    title = "{A composite Hertzsprung-Russell diagram for the peculiar red giants}",
    journal = {\apj},
    year = 1976,
    month = jun,
    volume = 206,
    pages = {474--489},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...206..474S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Scalo1978ApJ...225..523S,
    author = {{Scalo}, J.~M. and {Miller}, G.~E.},
    title = "{A constraint on proposed explanations for low $^{12}$C/$^{13}$C ratios in G-K giants}",
    journal = {\apj},
    year = 1978,
    month = oct,
    volume = 225,
    pages = {523--526},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...225..523S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Scargle1979ApJ...228..838S,
    author = {{Scargle}, J.\ D. and {Strecker}, D.\ W.},
    title = "Cool stars - Effective temperatures, angular diameters, and reddening determined from 1-5 micron flux curves and model atmospheres",
    journal = {\apj},
    year = 1979,
    month = mar,
    volume = 228,
    pages = {838--853},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...228..838S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Schaeidt1996A&A...315L..55S,
    author = {{Schaeidt}, S.\ G. and {Morris}, P.\ W. and {Salama}, A. and 
        {Vandenbussche}, B. and {Beintema}, D.\ A. and {Boxhoorn}, D.\ R. and 
        {Feuchtgruber}, H. and {Heras}, A.\ M. and {Lahuis}, F. and 
        {Leech}, K. and {Roelfsema}, P.\ R. and {Valentijn}, E.\ A. and 
        {Bauer}, O.\ H. and {van der Bliek}, N.\ S. and {Cohen}, M. and 
        {de Graauw}, T. and {Haser}, L.\ N. and {van der Hucht}, K.\ A. and 
        {Huygen}, E. and {Katterloher}, R.\ O. and {Kessler}, M.\ F. and 
        {Koornneef}, J. and {Luinge}, W. and {Lutz}, D. and {Planck}, M. and 
        {Spoon}, H. and {Waelkens}, C. and {Waters}, L.\ B.\ F.\ M. and 
        {Wieprecht}, E. and {Wildeman}, K.\ J. and {Young}, E. and {Zaal}, P.
        },
    title = {The photometric calibration of the ISO Short Wavelength Spectrometer.},
    journal = {\aap},
    year = 1996,
    month = nov,
    volume = 315,
    pages = {L55--L59},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...315L..55S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{Shipman2001clim.confE..18S,
    author = {{Shipman}, R.\ F. and {Morris}, P.\ W. and {Beintema}, D.\ A. and 
        {Boxhoorn}, D. and {Feuchtgruber}, H. and {Heras}, A.\ M. and 
        {Huygen}, R. and {Kester}, D. and {Lahuis}, F. and {Leech}, K. and 
        {Lorente}, R. and {Lutz}, D. and {Roelfsema}, P. and {Salama}, A. and 
        {Schaeidt}, S.\ G. and {Valentijn}, E. and {Vandenbussche}, B. and 
        {Wieprecht}, E.},
    title = "SWS In-flight Calibration",
    booktitle = {`The calibration legacy of the ISO Mission'},
    year = 2001,
    pages = {to be published},
      EDITOR    = {{Metcalfe}, L. and {Kessler}, M.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001clim.confE..18S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}





@BOOK{Seaton1995QB809.O63......,
    author = {{Seaton}, M.\ J.},
    title = {The opacity project},
    publisher = {Bristol, UK ; Philadelphia : Institute of Physics Pub.},
    year = 1995,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995QB809.O63......&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Smalley1993A&A...271..515S,
    author = {{Smalley}, B. and {Dworetsky}, M.\ M.},
    title = {The Atmospheric Parameters of A-Stars and F-Stars - Part One - Comparison of Various Methods},
    journal = {\aap},
    year = 1993,
    month = apr,
    volume = 271,
    pages = {515},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...271..515S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smalley1995A&A...293..446S,
    author = {{Smalley}, B. and {Dworetsky}, M.\ M.},
    title = {The calibration of uvby$\{$beta$\}$ photometry for B, A and F stars. I. Fundamental atmospheric parameters.},
    journal = {\aap},
    year = 1995,
    month = jan,
    volume = 293,
    pages = {446--456},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...293..446S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smalley1997A&A...328..349S,
    author = {{Smalley}, B. and {Kupka}, F.},
    title = "{The role of convection on the UVBY colours of A, F, and G stars}",
    journal = {\aap},
    year = 1997,
    month = dec,
    volume = 328,
    pages = {349--360},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...328..349S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1985ApJ...294..326S,
    author = {{Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = {The chemical composition of red giants. I - Dredge-up in the M and MS stars},
    journal = {\apj},
    year = 1985,
    month = jul,
    volume = 294,
    pages = {326--338},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985ApJ...294..326S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1986A&A...165..126S,
    author = {{Smith}, G. and {Edvardsson}, B. and {Frisk}, U.},
    title = "Non-resonance lines of neutral calcium in the spectra of the Alpha Centauri binary system",
    journal = {\aap},
    year = 1986,
    month = sep,
    volume = 165,
    pages = {126--134},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...165..126S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1986ApJ...311..843S,
    author = {{Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = {The chemical composition of red giants. II - Helium burning and the s-process in the MS and S stars},
    journal = {\apj},
    year = 1986,
    month = dec,
    volume = 311,
    pages = {843--863},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986ApJ...311..843S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1990ApJS...72..387S,
    author = {{Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = "The chemical composition of red giants. III - Further CNO isotopic and s-process abundances in thermally pulsing asymptotic giant branch stars",
    journal = {\apjs},
    year = 1990,
    month = feb,
    volume = 72,
    pages = {387--416},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJS...72..387S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1993A&A...274..335S,
    author = {{Smith}, K.\ C. and {Dworetsky}, M.\ M.},
    title = "Elemental Abundances in Normal Late B-Stars and Hgmn-Stars from Co-Added IUE Spectra - Part One - Iron Peak Elements",
    journal = {\aap},
    year = 1993,
    month = jul,
    volume = 274,
    pages = {335},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...274..335S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@PHDTHESIS{Sneden1974,
    author = {{Sneden}, C.},
    school = {University of Texas},
    year = 1974,
}


@INPROCEEDINGS{Sneden1991IAUS..145..235S,
    author = {{Sneden}, C.},
    title = "CNO Abundances of Stars Undergoing First Dredge up Mixing",
    booktitle = {IAU Symp. 145: Evolution of Stars: the Photospheric Abundance Connection},
    year = 1991,
    volume = 145,
    pages = {235},
    editor= {{Michaud}, G. and {Tutukov}, A.\ V.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991IAUS..145..235S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Soderblom1986A&A...158..273S,
    author = {{Soderblom}, D.\ R.},
    title = {The temperatures of Alpha Centauri A and B},
    journal = {\aap},
    year = 1986,
    month = apr,
    volume = 158,
    pages = {273},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...158..273S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sokolov1995A&AS..110..553S,
    author = {{Sokolov}, N.\ A.},
    title = {The determination of T\_eff\_ of B, A and F main sequence stars from the continuum between 3200 A and 3600 A.},
    journal = {\aaps},
    year = 1995,
    month = may,
    volume = 110,
    pages = {553},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26AS..110..553S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Spite1989A&A...210...25S,
    author = {{Spite}, F. and {Spite}, M. and {Francois}, P.},
    title = {Chemical evolution of the Magellanic Clouds. I - Metal abundance in three young supergiants of the Small Cloud},
    journal = {\aap},
    year = 1989,
    month = feb,
    volume = 210,
    pages = {25--34},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989A%26A...210...25S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Stencel1980ApJS...44..383S,
    author = {{Stencel}, R.\ E. and {Linsky}, J.\ L. and {Mullan}, D.\ J. and 
        {Basri}, G.\ S. and {Worden}, S.\ P.},
    title = "The outer atmospheres of cool stars. VII - High resolution, absolute flux profiles of the MG II H and K lines in stars of spectral types F8 to M5",
    journal = {\apjs},
    year = 1980,
    month = nov,
    volume = 44,
    pages = {383--402},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJS...44..383S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Sugar1985aeli.book.....S,
    author = {{Sugar}, J. and {Corliss}, C.},
    title = {Atomic energy levels of the iron-period elements: Potassium through Nickel},
    publisher = {Washington: American Chemical Society},
    year = 1985,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985aeli.book.....S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Taylor1999A&AS..134..523T,
    author = {{Taylor}, B.\ J.},
    title = "Catalogs of temperatures and [Fe/H] averages for evolved G and K stars",
    journal = {\aaps},
    year = 1999,
    month = feb,
    volume = 134,
    pages = {523--524},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26AS..134..523T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Tielens1983ApJ...271..702T,
    author = {{Tielens}, A.\ G.\ G.\ M.},
    title = "Stationary flows in the circumstellar envelopes of M giants",
    journal = {\apj},
    year = 1983,
    month = aug,
    volume = 271,
    pages = {702--716},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983ApJ...271..702T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tipping1981,
        AUTHOR  = {{Tipping}, R.\ H. and {Chackerian}, C.\ Jr.},
        TITLE   = "",
        YEAR    = 1981,
        JOURNAL = {J.\ Mol. Spectr.},
        VOLUME  = 88,
        PAGES   = "352"}


@ARTICLE{Tomkin1975ApJ...199..436T,
    author = {{Tomkin}, J. and {Lambert}, D.\ L. and {Luck}, R.\ E.},
    title = "The C-12/C-13 ratio in stellar atmospheres. IV - Eleven G and K type giants",
    journal = {\apj},
    year = 1975,
    month = jul,
    volume = 199,
    pages = {436--442},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975ApJ...199..436T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tomkin1976ApJ...210..694T,
    author = {{Tomkin}, J. and {Luck}, R.\ E. and {Lambert}, D.\ L.},
    title = "The 12C/13C ratio in stellar atmospheres. VII. 38 giants and supergiants.",
    journal = {\apj},
    year = 1976,
    month = dec,
    volume = 210,
    pages = {694--701},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...210..694T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Trimble1981QJRAS..22..361T,
    author = {{Trimble}, V. and {Bell}, R.\ A.},
    title = {Spectroscopic Determination of Stellar Masses - Mene Tekel Arcturus},
    journal = {\qjras},
    year = 1981,
    volume = 22,
    pages = {361},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981QJRAS..22..361T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tsuji1981A&A....99...48T,
    author = {{Tsuji}, T.},
    title = {Spectral energy distribution and effective temperature scale of M-giant stars. II - Application of the infra-red flux method},
    journal = {\aap},
    year = 1981,
    month = jun,
    volume = 99,
    pages = {48--57},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981A%26A....99...48T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Tsuji1986A&A...156....8T,
    author = {{Tsuji}, T.},
    title = "High resolution spectroscopy of CO in the infrared spectra of cool stars - Turbulent velocities and carbon abundance in M-giant stars",
    journal = {\aap},
    year = 1986,
    month = feb,
    volume = 156,
    pages = {8--21},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...156....8T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tsuji1991A&A...245..203T,
    author = {{Tsuji}, T.},
    title = "High resolution spectroscopy of CO in the infrared spectra of cool stars. III - Line intensities, shifts, and asymmetries as probes of stellar turbulence and abundance in oxygen-rich giants",
    journal = {\aap},
    year = 1991,
    month = may,
    volume = 245,
    pages = {203--218},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...245..203T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Tsuji1994A&A...289..469T,
    author = {{Tsuji}, T. and {Ohnaka}, K. and {Hinkle}, K.\ H. and {Ridgway}, S.\ T.
        },
    title = "High resolution infrared spectra of silicon monoxide and silicon isotopic abundances in cool luminous stars",
    journal = {\aap},
    year = 1994,
    month = sep,
    volume = 289,
    pages = {469--491},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...289..469T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tsuji1997A&A...320L...1T,
    author = {{Tsuji}, T. and {Ohnaka}, K. and {Aoki}, W. and {Yamamura}, I.
        },
    title = {Warm molecular envelope of M giants and Miras: a new molecule forming region unmasked by the ISO SWS.},
    journal = {\aap},
    year = 1997,
    month = apr,
    volume = 320,
    pages = {L1--L4},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...320L...1T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Vandenbussche1999,
        AUTHOR  = "{Vandenbussche}, B.",
        TITLE   = {The ISO-SWS Relative Spectral Response Calibration},
      PUBLISHER = {ISO-SWS online documentation},
        YEAR    = 1999}



@INPROCEEDINGS{Vandenbussche2001clim.confE..97V,
    author = {{Vandenbussche}, B. and {Morris}, P.~W. and {Valentijn}, E.~A. and 
        {Beintema}, D.~A. and {Boxhoorn}, D.~R. and {Decin}, L. and 
        {Feuchtgruber}, H. and {Heras}, A.~M. and {Lahuis}, F. and {Lorente}, R. and 
        {Lutz}, D. and {Roelfsema}, P.~R. and {Salama}, A. and {Schaeidt}, S.~G. and 
        {Shipman}, R.~F. and {Spoon}, H.~W.~W. and {van Malderen}, R. and 
        {Waters}, L.~B.~F.~M. and {Wieprecht}, E. and {Zaal}, P.},
    title = "{The Relative Spectral Response Calibration of the ISO-SWS}",
    booktitle = {The Calibration Legacy of the ISO Mission},
    year = 2001,
    pages = {97},
      EDITOR    = {{Metcalfe}, L. and {Kessler}, M.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001clim.confE..97V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{Vanhoof1998sese.conf...67V,
    author = {{van Hoof}, P.\ A.\ M.},
    title = {A comprehensive line list for atomic transitions on the WWW},
    booktitle = {Stellar Evolution, Stellar Explosions and Galactic Chemical Evolution},
    year = 1998,
    pages = {67},
      EDITOR    = {{Mezzacappa}, A.},
        ADDRESS = "Institute of Physics Publishing"}

@ARTICLE{vanParadijs1973A&A....23..369V,
    author = {{van Paradijs}, J.},
    title = "An analysis of the line spectra of some G and K Ib supergiants.",
    journal = {\aap},
    year = 1973,
    month = mar,
    volume = 23,
    pages = {369},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1973A%26A....23..369V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{vanParadijs1974A&A....35..225V,
    author = {{van Paradijs}, J. and {Meurs}, E.\ J.\ A.},
    title = "A differential abundance analysis of alpha Tau relative to alpha Boo",
    journal = {\aap},
    year = 1974,
    month = oct,
    volume = 35,
    pages = {225--231},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974A%26A....35..225V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{vanParadijs1976A&A....53....1V,
    author = {{van Paradijs}, J. and {Kester}, D.},
    title = "{Abondances of carbon, nitrogen and oxygen in six G and K type giants.}",
    journal = {\aap},
    year = 1976,
    month = nov,
    volume = 53,
    pages = {1--8},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976A%26A....53....1V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Venn1990ApJ...363..234V,
    author = {{Venn}, K.\ A. and {Lambert}, D.\ L.},
    title = "The chemical composition of three Lambda Bootis stars",
    journal = {\apj},
    year = 1990,
    month = nov,
    volume = 363,
    pages = {234--244},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJ...363..234V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Volk1989AJ.....98.1918V,
    author = {{Volk}, K. and {Cohen}, M.},
    title = {On the calibration of the IRAS low-resolution spectra},
    journal = {\aj},
    year = 1989,
    month = nov,
    volume = 98,
    pages = {1918--1934},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989AJ.....98.1918V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Wallace1995Sci...268.1155W,
    author = {{Wallace}, L. and {Bernath}, P. and {Livingston}, W. and {Hinkle}, K. and 
        {Busler}, J. and {Guo}, B. and {Zhang}, K.},
    title = "Water on the Sun",
    journal = {Science},
    year = 1995,
    month = may,
    volume = 268,
    pages = {1155},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995Sci...268.1155W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Wamsteker1981A&A....97..329W,
    author = {{Wamsteker}, W.},
    title = "{Standard stars and calibration for JHKLM photometry}",
    journal = {\aap},
    year = 1981,
    month = apr,
    volume = 97,
    pages = {329--333},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981A%26A....97..329W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Wiese1966atp..book.....W,
    author = {{Wiese}, W.\ L. and {Smith}, M.\ W. and {Glennon}, B.\ M.},
    title = {Atomic transition probabilities. Vol.: Hydrogen through Neon. A critical data compilation},
    publisher = {NSRDS-NBS 4, Washington},
    year = 1966,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1966atp..book.....W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Wiese1969atp..book.....W,
    author = {{Wiese}, W.\ L. and {Smith}, M.\ W. and {Miles}, B.\ M.},
    title = {Atomic transition probabilities. Vol. 2: Sodium through Calcium. A critical data compilation},
    publisher = {NSRDS-NBS 22, Washington},
    year = 1969,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1969atp..book.....W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Wilson1976ApJ...205..823W,
    author = {{Wilson}, O.~C.},
    title = "{Absolute magnitudes of stars from widths of chromospheric CaII emission lines.}",
    journal = {\apj},
    year = 1976,
    month = may,
    volume = 205,
    pages = {823--840},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...205..823W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Witteborn1999AJ....117.2552W,
    author = {{Witteborn}, F.\ C. and {Cohen}, M. and {Bregman}, J.\ D. and 
        {Wooden}, D.\ H. and {Heere}, K. and {Shirley}, E.\ L.},
    title = {Spectral Irradiance Calibration in the Infrared. XI. Comparison of alpha Bootis and 1 Ceres with a Laboratory Standard},
    journal = {\aj},
    year = 1999,
    month = may,
    volume = 117,
    pages = {2552--2560},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999AJ....117.2552W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Woitke1999A&A...348L..17W,
    author = {{Woitke}, P. and {Helling}, C. and {Winters}, J.\ M. and {Jeong}, K.\ S.
        },
    title = "On the formation of it warm molecular layers",
    journal = {\aap},
    year = 1999,
    month = aug,
    volume = 348,
    pages = {L17--L20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...348L..17W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Worthey1994ApJS...95..107W,
    author = {{Worthey}, G.},
    title = "Comprehensive stellar population models and the disentanglement of age and metallicity effects",
    journal = {\apjs},
    year = 1994,
    month = nov,
    volume = 95,
    pages = {107--149},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994ApJS...95..107W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Worthey1994ApJS...94..687W,
    author = {{Worthey}, G. and {Faber}, S.~M. and {Gonzalez}, J.~J. and {Burstein}, D.
        },
    title = "{Old stellar populations. 5: Absorption feature indices for the complete LICK/IDS sample of stars}",
    journal = {\apjs},
    year = 1994,
    month = oct,
    volume = 94,
    pages = {687--722},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994ApJS...94..687W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Yamamura1999A&A...341L...9Y,
    author = {{Yamamura}, I. and {de Jong}, T. and {Onaka}, T. and {Cami}, J. and 
        {Waters}, L.\ B.\ F.\ M.},
    title = "Detection of warm SO\_2 gas in oxygen-rich AGB stars",
    journal = {\aap},
    year = 1999,
    month = jan,
    volume = 341,
    pages = {L9--L12},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...341L...9Y&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Zahn1992A&A...265..115Z,
    author = {{Zahn}, J.\ -.},
    title = "Circulation and turbulence in rotating stars",
    journal = {\aap},
    year = 1992,
    month = nov,
    volume = 265,
    pages = {115--132},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...265..115Z&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



